AdaptSR: Low-Rank Adaptation for Efficient and Scalable Real-World Super-Resolution

Recovering high-frequency details and textures from low-resolution images remains a fundamental challenge in super-resolution (SR), especially when real-world degradations are complex and unknown. While GAN-based methods enhance realism, they suffer from training instability and introduce unnatural artifacts. Diffusion models, though promising, demand excessive computational resources, often requiring multiple GPU days, even for single-step variants. Rather than naively fine-tuning entire models or adopting unstable generative approaches, we introduce AdaptSR, a low-rank adaptation (LoRA) framework that efficiently repurposes bicubic-trained SR models for real-world tasks. AdaptSR leverages architecture-specific insights and selective layer updates to optimize real SR adaptation. By updating only lightweight LoRA layers while keeping the pretrained backbone intact, it captures domain-specific adjustments without adding inference cost, as the adapted layers merge seamlessly post-training. This efficient adaptation not only reduces memory and compute requirements but also makes real-world SR feasible on lightweight hardware. Our experiments demonstrate that AdaptSR outperforms GAN and diffusion-based SR methods by up to 4 dB in PSNR and 2% in perceptual scores on real SR benchmarks. More impressively, it matches or exceeds full model fine-tuning while training 92% fewer parameters, enabling rapid adaptation to real SR tasks within minutes.

==> sec/4_experiments_cvpr.tex <==
\begin{figure}
\centering
\input{images/training_time_vs_psnr_ft_vs_lora} \vspace{-0.5cm}
\caption{Number of iterations vs. performance comparison for full model finetuning and LoRA-enhanced models for SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially}. LoRA reaches peak PSNR in just 100k iterations, completing in 4 hours for SwinIR and 1 hours for SAFMN on an NVIDIA RTX 4090, whereas fine-tuning takes significantly longer—23 hours for SwinIR and 9 hours for SAFMN—to achieve similar performance. The dashed lines of LoRA methods indicate their final PSNR performance at their latest iteration 100k.}
\label{fig:numiter_vs_psnr}
\end{figure}


\section{Experiments}
\subsection{Experimental Settings}
\noindent
\textbf{Datasets.}
We train AdaptSR on DIV2K \cite{Agustsson_2017_CVPR_Workshops} and RealSR \cite{realsr_cai2019toward} training sets, using the Real-ESRGAN \cite{wang2021real} degradation pipeline to create LR-HR pairs. During training, we also utilize the DIV2K unknown degradation dataset to cover a wider range of degradation types, using randomly cropped $256\times256$ patches from the HR images. For evaluation, we benchmark against other methods on DIV2K \cite{Agustsson_2017_CVPR_Workshops}, RealSR \cite{realsr_cai2019toward}, and DRealSR \cite{drealsr_wei2020component} test sets. Especially to compare with diffusion-based approaches, we adopt the StableSR \cite{wang2024exploiting} validation setup, including 3000 patches from DIV2K, 100 from RealSR, and 93 from DRealSR, with LR-HR pairs sized at $128\times128$ and $512\times512$.

\noindent
\textbf{Implementation Details and Evaluation.}
All experiments were run on an NVIDIA Quadro RTX 4090 GPU using PyTorch. LoRA models rank 8 with \( \alpha \) value 1 were trained for 100k iterations with Adam \cite{kingma2014adam} and L1 loss, starting with a learning rate of $1e^{-3}$, reduced by 25$\%$ at 50k, 75k, and 90k iterations. In comparison, full model fine-tuning required 500k iterations to achieve comparable results, with the learning rate halved at 250k, 400k, 450k and 475k intervals. Both LoRA and fine-tuning used the same settings, including the Adam optimizer \cite{kingma2014adam}, a batch size of 8, and the L1 loss function. To evaluate fidelity and perceptual quality, we used PSNR and SSIM (Y channel in YCbCr space) and perceptual metrics LPIPS \cite{lpips} and DISTS \cite{dists}.


% All experiments were conducted on an NVIDIA Quadro RTX 4090 GPU using the PyTorch framework. We trained all LoRA models for 100k iterations with the Adam optimizer \cite{kingma2014adam} and L1 loss function, using a mini-batch size of 8 and an initial learning rate of $1e^{-3}$. The learning rate was decreased by 25$\%$ at the 50k, 75k, and 90k iterations. In contrast, full model fine-tuning on Tesla V100 GPU required 500k iterations with the learning rate halved at 250k, 400k, 450k and 475k iterations. For finetuning experiments, we used the same settings as for the LoRA models; an initial learning rate of $1e^{-3}$, a mini-batch size of 8, and the Adam optimizer \cite{kingma2014adam} with the L1 loss function.

% To comprehensively assess the performance of our LoRA methods and other state-of-the-art GAN-based and diffusion-based real SR methods, we use both full-reference and no-reference metrics. PSNR and SSIM (computed on the Y channel in YCbCr space) serve as fidelity metrics with ground-truth reference, while LPIPS \cite{lpips} and DISTS \cite{dists} measure perceptual quality. For no-reference quality assessment, we employ NIQE \cite{niqe_zhang2015feature}, MUSIQ \cite{ke2021musiq}, MANIQA \cite{yang2022maniqa} and CLIPIQA \cite{clipiqa_wang2022exploring}.

\subsection{AdaptSR vs. Fine-Tuning}
\label{sec:fine}
Table \ref{table:diff_degredation_lora} presents the performance of bicubic-trained SR models, their fine-tuned counterparts, and LoRA-based adaptations on the RealSR dataset \cite{realsr_cai2019toward}. LoRA consistently delivers comparable or superior results to fine-tuning with far less memory and compute requirements. For example, in SwinIR \cite{liang2021swinir}, LoRA improves PSNR by 0.42 dB, SSIM by 2$\%$, and LPIPS by 3.2$\%$ using only 886k parameters versus 12M required for fine-tuning. In SAFMN \cite{safmn_sun2023spatially}, LoRA achieves similar gains while updating around 100k parameters—half of what fine-tuning requires. Importantly, since LoRA layers merge into the base model post-training, inference speeds remain unaffected. 

Across various architectures, LoRA adaptation enhances both fidelity and perceptual quality, with models seeing up to a 1 dB PSNR boost and a 4$\%$ SSIM improvement over bicubic baselines. Specifically, SwinIR+LoRA gains 1.14 dB in PSNR and 4.4$\%$ in SSIM on RealSR \cite{realsr_cai2019toward}. Perceptual metrics like LPIPS \cite{lpips} and DISTS \cite{dists} show reductions in artifacts and improved visual quality (see Sec. \ref{sec:comparison}). Additionally, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA achieves rapid convergence—100k iterations, or approximately 4 hours on SwinIR and 1 hours on SAFMN using an NVIDIA RTX 4090—compared to 23 and 9 hours, respectively, for fine-tuning. These results highlight efficiency and high performance of LoRA adaptation as a fine-tuning alternative, offering strong fidelity and perceptual quality with minimal training time.

 % Table \ref{table:diff_degredation_lora} summarizes the performance of SoTA CNN and Transformer-based SR models adapted from bicubic to real-world SR using LoRA layers versus standard fine-tuning on RealSR \cite{realsr_cai2019toward} dataset. Clearly, LoRA delivers similar or better performance than fine-tuning with significantly less memory and computational cost. For SwinIR \cite{liang2021swinir}, LoRA boosts PSNR by 0.42 dB, SSIM by 2$\%$, and LPIPS by 3.2$\%$ while updating only 886k parameters versus 12M for fine-tuning. For lightweight SAFMN \cite{safmn_sun2023spatially}, LoRA achieves similar gains with just around 100k parameters which is half of the parameters required for fine-tuning. Crucially, since LoRA layers are merged into the base model post-training, inference speed remains unchanged. Furthermore, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA converges within 100k iterations, taking 5 hours on SwinIR and 2.5 hours on SAFMN on an NVIDIA RTX 4090, compared to 4 days and 1 day, respectively, for fine-tuning. These results highlight efficiency and high performance of LoRA adaptation as a fine-tuning alternative, offering strong fidelity and perceptual quality with minimal training time.
 
% Table \ref{table:diff_degredation_lora} presents a comparison between LoRA-based adaptation and standard fine-tuning for $\times$4 real super-resolution on SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially} using the RealSR validation set\cite{realsr_cai2019toward}. Clearly, LoRA delivers similar or better performance than fine-tuning with significantly less memory and computational cost. For SwinIR \cite{liang2021swinir}, LoRA boosts PSNR by 0.42 dB, SSIM by 2$\%$, and LPIPS by 3.2$\%$ while updating only 886k parameters versus 12M for fine-tuning. For lightweight SAFMN \cite{safmn_sun2023spatially}, LoRA achieves similar gains with just around 100k parameters which is half of the parameters required for fine-tuning. Crucially, since LoRA layers are merged into the base model post-training, inference speed remains unchanged. Furthermore, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA converges within 100k iterations, taking 5 hours on SwinIR and 2.5 hours on SAFMN on an NVIDIA RTX 4090, compared to 4 days and 1 day, respectively, for fine-tuning. These results highlight efficiency and high performance of LoRA adaptation as a fine-tuning alternative, offering strong fidelity and perceptual quality with minimal training time.


\begin{table}
 \caption{\textit{Performance comparison for domain adaptation between fine-tuning and LoRA-enhanced models} on RealSR \cite{realsr_cai2019toward}. LoRA matches or outperforms standard fine-tuning with significantly fewer trainable parameters and shorter training time, while maintaining the inference speed of baseline models. Here, $^{*}$ denotes the bicubic-trained model.}
    \centering
    \scalebox{0.7}{
    \begin{tabular}{ccccccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{Model} & Trainable & FLOPs & GPU & \multirow{2}{*}{PSNR} & \multirow{2}{*}{SSIM} & \multirow{2}{*}{LPIPS}\\
     & Parameters & (G) & Hours &  & & \\  
    \hline
    EDSR$^{*}$ & 1.5M & - & - &27.5422 & 0.7732 & 0.3937\\
     +FineTuning & +1.5M & 64.97 & 10 & 28.0605& 0.7963& 0.3203 \\
     + LoRA & +314k & 54.76 & 1.05 & 27.9260 & 0.7878 & 0.2835 \\
     \hdashline
    SAFMN$^{*}$ & 240k & - & - & 27.5383 & 0.7740 & 0.3927 \\
     + FineTuning & +240k & 7.75 & 9 &28.3173 & 0.7936 & 0.2887  \\
     + LoRA & +99.5k & 5.89 & 1.17 & 28.3245 & 0.7935 & 0.2935  \\ 
     \hdashline
    SwinIR$^{*}$ & 12M  & - & - & 27.5537 & 0.7738 & 0.3965\\
     + FineTuning & +12M & 428.41 & 23 & 28.2537 & 0.7906 & 0.3820 \\
     + LoRA & +886k & 410.57 & 4 & 28.6964 & 0.8079 & 0.2591  \\ 
     \hdashline
    DRCT$^{*}$ & 14M & - & - & 27.5502 & 0.7737 & 0.3966  \\ 
     + FineTuning & +14M & 594.64 & 32 & 28.7481& 0.8100& 0.3007 \\
     + LoRA & +3M & 482.72 & 5.45 & 28.7173 & 0.8061 & 0.2553\\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_degredation_lora}
\end{table}


% Table \ref{table:diff_degredation_lora} compares LoRA-based adaptation with standard fine-tuning for $\times$4 SR on Transformer-based SwinIR \cite{liang2021swinir} and CNN-based SAFMN \cite{safmn_sun2023spatially}, evaluated on the DIV2K unknown validation set \cite{Agustsson_2017_CVPR_Workshops}. LoRA delivers comparable or superior performance to fine-tuning while significantly reducing memory and computational demands. For SwinIR, LoRA improves PSNR by 0.75 dB, SSIM by $2.5\%$, and LPIPS by $5.8\%$ while updating only 886k parameters ($8\%$ of total) compared to 12M for fine-tuning. For SAFMN, LoRA achieves similar results with only 100k updated parameters—half the amount required by fine-tuning. Crucially, since LoRA layers are merged into the base model post-training, inference speed remains unchanged. Furthermore, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA converges within 100k iterations, requiring just 5 hours for SwinIR and 2.5 hours for SAFMN on an NVIDIA RTX 4090, compared to 4 days and 1 day for fine-tuning, respectively. These results highlight LoRA adapted approaches as a memory-efficient, high-performance alternative to fine-tuning, providing strong fidelity and perceptual quality with minimal training overhead.
%Table \ref{table:diff_degredation_lora} compares LoRA-based adaptation with standard fine-tuning on the $\times$4 SR task using SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially} models, evaluated on the DIV2K unknown validation set \cite{Agustsson_2017_CVPR_Workshops}. LoRA achieves comparable or superior results to fine-tuning while greatly reducing memory and computational costs for both baseline models. Specifically, for SwinIR \cite{liang2021swinir}, LoRA surpasses fine-tuning by 0.75 dB in PSNR, $2.5\%$ in SSIM, and $5.8\%$in LPIPS, while updating only 886k parameters ($8\%$ of all parameters) compared to 12M for fine-tuning. For the lightweight SAFMN \cite{safmn_sun2023spatially} model, LoRA achieves comparable performance to fine-tuning while updating only 100k parameters—half the number required by fine-tuning. Importantly, since LoRA layers are merged into the base model after training, inference speed remains the same as the original model. As shown in Figure \ref{fig:numiter_vs_psnr}, LoRA reaches peak PSNR within 100k iterations, requiring only 5 hours and 2.5 hours on an NVIDIA RTX 4090, for SwinIR and SAFMN, respectively. On the other hand, fine-tuning SwinIR takes 4 days and SAFMN requires 1 day to achieve comparable performance. These results confirm that LoRA is a high-performance, memory-efficient alternative to fine-tuning, offering strong fidelity and perceptual quality with minimal training overhead.

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/training_time_vs_psnr_ft_vs_lora}
% \caption{Number of iterations vs. performance comparison for full model finetuning and LoRA-enhanced models for SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially}. LoRA reaches peak PSNR in just 100k iterations, completing in 5 hours for SwinIR and 2.5 hours for SAFMN on an NVIDIA RTX 4090, whereas fine-tuning takes significantly longer—4 days for SwinIR and 1 day for SAFMN—to achieve similar performance.}
% \label{fig:numiter_vs_psnr}
% \end{figure}



% \begin{table*}
%  \caption{Performance comparison of SR models for domain adaptation from bicubic to real SR. LoRA-enhanced models consistently improve fidelity and perceptual quality over baseline methods with minimal additional parameters.}
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{ccccccccc}
%     \specialrule{.1em}{.05em}{.05em} 
%      Metric & EDSR & EDSR+LoRA & SAFMN & SAFMN+LoRA & SwinIR & SwinIR+LoRA & DRCT & DRCT+LoRA \\ 
%      & & +300k & & +99.5k & & +886k & & +3M \\
%      \hline
%      PSNR $\uparrow$ & 27.5422& 27.9260& 27.5583& 28.3245& 27.5537& 28.6964& 27.5502& 28.7173\\
%      SSIM $\uparrow$ &  0.7732 & 0.7878 & 0.7740 & 0.7935 & 0.7738 & 0.8079 & 0.7737 & 0.8061 \\
%      LPIPS $\downarrow$ &  0.3937&0.2835&0.3927&0.2935&0.3965&0.2591&0.3966&0.2553 \\
%      DISTS $\downarrow$ &  0.2436&0.2190&0.2430&0.2229&0.2426&0.2109&0.2434&0.2094 \\ 
%      % CLIPIQA$\uparrow$& 0.3289&0.2829&0.3338&0.2614&0.3388&0.3264&0.3384&0.3206\\
%      % NIQE$\downarrow$ &  8.3179&7.8546&8.3443&7.7209&8.3294&8.3661&8.3130&8.3144 \\
%      % MUSIQ$\uparrow$ & 30.8765&43.9013&30.7043&41.8672&30.5589&48.4967&30.5884&48.0846 \\
%      %  MANIQA $\uparrow$ &  0.3642 & 0.3766 & 0.3703 & 0.3780 & 0.3711 & 0.3947 & 0.3671 & 0.3968 \\
% \specialrule{.1em}{.05em}{.05em} 
%     \end{tabular} 
% }
% \label{table:domain_adaptation}
% \end{table*}

% \subsection{Bicubic to Real SR with LoRA}
% Table \ref{table:domain_adaptation} summarizes the performance of SoTA CNN and Transformer-based SR models adapted from bicubic to real-world SR using LoRA layers. Across models including EDSR \cite{EDSR2017}, SAFMN \cite{safmn_sun2023spatially}, SwinIR \cite{liang2021swinir}, and DRCT \cite{drct_Hsu_2024_CVPR}, LoRA adaptation significantly enhances both fidelity and perceptual quality. LoRA models achieve up to a 1 dB PSNR boost and a 4$\%$ SSIM increase for all models compared to their bicubic baselines. Specifically, SwinIR+LoRA notably gains 1.14 dB in PSNR and 4.4$\%$ in SSIM over bicubic-trained models on the RealSR \cite{realsr_cai2019toward} dataset. Perceptual metrics like LPIPS \cite{lpips} and DISTS \cite{dists} also indicate reduced artifacts and improved visual quality, as detailed in Sec. \ref{sec:qual}. This demonstrates the effectiveness of LoRA in achieving efficient domain adaptation for real-world SR neither requiring long hours of GPU training nor sacrificing the inference speed and perceptual quality.


 
%Table \ref{table:domain_adaptation} presents the performance of various SR models adapted from bicubic training to real-world SR using LoRA layers. Across all tested models; EDSR \cite{EDSR2017}, SAFMN \cite{safmn_sun2023spatially}, SwinIR \cite{liang2021swinir} and DRCT \cite{drct_Hsu_2024_CVPR}, training LoRA layers for domain adaptation significantly boosts both fidelity and perceptual quality. In terms of PSNR and SSIM, LoRA-enhanced models consistently outperform their baseline counterparts, with improvements of up to 1 dB in PSNR and noticeable gains of 4$\%$ in SSIM. For instance, SwinIR+LoRA improves baseline PSNR performance by 1.14 dB and SSIM performance by 4.4$\%$. Moreover, these improvements extend to perceptual metrics as well. LoRA-enhanced models exhibit lower LPIPS \cite{lpips} and DISTS \cite{dists} scores, indicating a reduction in perceptual artifacts and an overall improvement in visual quality. Importantly, since LoRA layers are merged with the base model after training, the inference time remains identical to the baseline while maintaining computational efficiency. This demonstrates the effectiveness of LoRA in achieving efficient domain adaptation for real-world SR neither requiring long hours of GPU training nor sacrificing the inference speed.

\subsection{Module-wise Importance for Adaptation}
\label{sec:adapt}
% To determine the most critical modules for domain adaptation from bicubic to real SR, we applied LoRA to specific components in SwinIR \cite{liang2021swinir} in four configurations: (1) all layers (convolutional, linear, and attention layers), (2) only convolutional layers, (3) only multi-head self-attention (MSA) layers, and (4) only MLP layers. Figure \ref{fig:training_time_vs_psnr} compares training time and PSNR for these configurations over 10k iterations. Applying LoRA across all layers achieved full fine-tuning performance in just 50 minutes (vs. 4 days), with only 8$\%$ of parameters. LoRA applied to convolutional layers alone, with just 2$\%$ of parameters, reached near full-tuning performance within 30 minutes. Notably, LoRA models began at a PSNR of 22.606 dB, matching the bicubic baseline's initial performance. 
To identify the crucial modules for adapting SwinIR \cite{liang2021swinir} from bicubic to real SR, we tested LoRA on four configurations: (1) all layers (convolutional, linear, and attention), (2) only convolutional layers, (3) only multi-head self-attention (MSA) layers, and (4) only MLP layers. As illustrated in Figure \ref{fig:training_time_vs_psnr}, applying LoRA to all layers achieved full fine-tuning results in just 50 minutes (compared to 23 hours), using only 8$\%$ of the original parameters. Focusing solely on convolutional layers achieved comparable performance within 30 minutes with only 2$\%$ of parameters. Notably, all configurations began at 22.606 dB PSNR, matching the initial bicubic baseline.

% Local attribution maps (LAM) \cite{lam_gu2021interpreting} are used to visualize the contribution of model components to feature interactions and contextual understanding. As shown in Figure \ref{fig:saliency_image}, LAM demonstrates that combining LoRA layers enhances these interactions compared to individual sub-modules or full model fine-tuning. 


Local Attribution Maps (LAM) \cite{lam_gu2021interpreting} visualize the contributions of components to feature interactions and context. Figure \ref{fig:saliency_image} shows that combining LoRA layers enhances these interactions beyond individual modules or full fine-tuning. Diffusion index (DI) \cite{lam_gu2021interpreting} values, indicating attention range, confirm that LoRA applied to all layers achieves the widest attention and strongest reconstruction and it is followed closely by the convolution-only LoRA performance. Remarkably, MLP-only and attention-only LoRA methods still surpass standard fine-tuning in capturing more features. This module analysis shows that LoRA in all layers is optimal for adaptation, with minimal parameter overhead, while focusing solely on convolutional layers (2$\%$ parameters) offers a highly efficient alternative to all layer adaptation. \textit{Additional module-wise analysis for other architectures are included in the supplementary.}

\begin{figure}
    \centering
    \input{images/training_time_vs_psnr_for_lora_modules.tex} \vspace{-0.5cm}
\caption{Training time vs. performance comparison for different LoRA modules with 10k iterations on DIV2K unknown \cite{Agustsson_2017_CVPR_Workshops}. The dashed line indicates the best PSNR achieved by standard fine-tuning, which requires 4 days of training. Notably, LoRA applied to all layers reaches this PSNR level in just 30 minutes.}
\label{fig:training_time_vs_psnr}
\end{figure}

\begin{table}
 \caption{\textit{Layer-wise importance for LoRA domain adaptation} from bicubic to real SR on DRealSR \cite{drealsr_wei2020component} dataset for rank 32.}
    \centering
    \scalebox{0.75}{
    \begin{tabular}{cccccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{LoRA Layer} & \multirow{2}{*}{PSNR} & \multirow{2}{*}{SSIM} & \multirow{2}{*}{LPIPS} & Trainable &  Training \\
    & & & & Parameters & Time (Mins)\\ 
    \hline
   MSAs  & 30.7712 & 0.8402 & 0.4023 & 1.2M & 77 \\
   MLPs  & 31.0241 & 0.8433 & 0.3999 & 1.2M & 57.71 \\
    All Convs & 30.9736 & 0.8425 & 0.3994 & 868k & 31.45 \\
   \hdashline
   First Conv & 30.0777 & 0.8226 & 0.4327 & 53k & 24.95 \\
   RSTLB Convs & 30.9682 & 0.8422 & 0.4003 & 622k & 41.09 \\
   DFE Convs & 29.5300 & 0.8088 & 0.4470 & 104k & 19.22 \\
   BU Conv & 29.5828 & 0.8117 & 0.4379 & 70k & 19.02  \\
   AU Conv & 30.4789 & 0.8305 & 0.4201 & 19k & 18.42 \\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:effect_of_lora_layers}
\end{table}

\begin{figure}
\centering
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/position_pil_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{Nikon 41 \\ DI \cite{lam_gu2021interpreting}}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/fine-tuned_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{SwinIR \cite{liang2021swinir} FT \\  16.08}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_attn_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{Attention Blocks \\ 14.72}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_mlp_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{MLP Blocks \\ 17.27}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_all_convs_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{Conv Layers \\ 18.78}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/all_lora_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{All Layers \\ 19.59}
\end{subfigure}
\caption{Comparison of \textbf{local attribution maps} (LAMs) \cite{lam_gu2021interpreting} between different LoRA modules and standard fine-tuning model on RealSR-Nikon41  \cite{realsr_cai2019toward} image. The LAM results denote the importance of each pixel in the input image when super-resolving the patch marked with a red box. The diffusion index (DI) \cite{lam_gu2021interpreting} value reflects the range of involved pixels hence better reconstruction.} \vspace{-0.5cm}
\label{fig:saliency_image} 
\end{figure} 

\begin{table*}[t!]
 \caption{\textit{Quantitative comparison of our proposed Low-Rank adaptation with the state-of-the-art real-world GAN and diffusion methods}. Our LoRA-enhanced approach trained only by L1 loss achieves high PSNR and SSIM scores while also delivering perceptual scores comparable to GAN and diffusion-based methods trained with perceptual losses. The best and the second-best results of each metric are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.}
    \centering
    \scalebox{0.7}{
    \begin{tabular}{c|l|cccc|ccccccc|c}
    \specialrule{.1em}{.05em}{.05em} 
    & & \multicolumn{4}{|c|}{GAN-based Real SR} & \multicolumn{7}{c|}{Diffusion-based Real SR} & \multicolumn{1}{c}{} \\
    \hline
    & & RealESRGAN & LDL & DASR & Real-SAFMN-L & StableSR & DiffBIR & ResShift & SeeSR & PASD & SinSR & OSEDiff & AdaptSR-T \\
    & & \cite{wang2018esrgan} & \cite{liang2022details} & \cite{liang2022efficient} & \cite{safmn_sun2023spatially} & \cite{wang2024exploiting} & \cite{rebuttal_lin2025diffbir} & \cite{yue2023resshift} & \cite{lora_diff_realsr_wu2024seesr} & \cite{yang2023pasd} & \cite{wang2024sinsr} & \cite{lora_diff_realsr_wu2024one} & (Ours) \\ 
    \hline
     \multirow{2}{*}{\centering Dataset} & Trainable & \multirow{2}{*}{\centering 17M} & \multirow{2}{*}{\centering 12M} & \multirow{2}{*}{\centering M} & \multirow{2}{*}{\centering 5.6M}& \multirow{2}{*}{\centering 150M} & \multirow{2}{*}{\centering 380M} & \multirow{2}{*}{\centering 118.6M} & \multirow{2}{*}{\centering 750M} & \multirow{2}{*}{\centering 625M} & \multirow{2}{*}{\centering 119M}& \multirow{2}{*}{\centering 8.5M}& \multirow{2}{*}{\centering 886k} \\
    & Parameters & & & & & & & & & & & \\
    \hline
    \multirow{4}{*}{\centering DIV2K} & PSNR $\uparrow$ & 22.94 & 23.76 & 21.72 & 23.21 & 23.68 & 20.84 & 20.94 & 21.75 & 23.14 & 24.41 & 23.72 & \textcolor{red}{25.81} \\
    & SSIM $\uparrow$ &  0.6036 &  0.6403&  0.5535 & 0.5950& 0.4887 & 0.4938 & 0.5422 & 0.6043 &  0.5505 &  0.6018 &  0.6108 & \textcolor{blue}{0.6681}\\
    & LPIPS $\downarrow$ &  0.3768 & \textcolor{blue}{0.3091}& 0.4266 &  0.3282& 0.4055 & 0.4270 & 0.4284 & 0.3194 &  0.3571 &  0.3240 &  \textcolor{red}{0.2941} & 0.5047 \\
    & DISTS $\downarrow$ &  0.2520&  0.2189& 0.2688 & 0.2153& 0.2542 & 0.2471 & 0.2606 & \textcolor{red}{0.1968}&  0.2207&  0.2066&  \textcolor{blue}{0.1976} & 0.3194\\
    \hline
    \multirow{4}{*}{\centering RealSR} & PSNR $\uparrow$ & 25.69 & 24.96 & 27.02 & 24.23 & 24.70 & 24.77 & 26.31 & 25.18 & 25.21 & 26.28 & 25.15 & \textcolor{blue}{28.70} \\
    & SSIM $\uparrow$ &  0.7616 &  0.7634& 0.7708 & 0.7217& 0.7085 & 0.6572 & 0.7421 &  0.7216&  0.6798&  0.7347&  0.7341& \textcolor{red}{0.8079} \\
    & LPIPS $\downarrow$ &  0.2727 & \textcolor{red}{0.2519}& 0.3151 &  0.2905& 0.3018 & 0.3658 & 0.3460 & 0.3009&  0.3380&  0.3188&  0.2921&  0.2591\\
    & DISTS $\downarrow$ &  \textcolor{blue}{0.2063}& \textcolor{red}{0.1981}& 0.2207 &  0.2176& 0.2135 & 0.2310 & 0.2498 &  0.2223&  0.2260&  0.2353&  0.2128&  0.2109 \\
     \hline
    \multirow{4}{*}{\centering DRealSR} & PSNR $\uparrow$ & 28.64 & 27.43 & 29.77 & 27.15 & 28.13 & 26.76 & 28.46 & 28.17 & 27.36 & 28.36 & 27.92 & 30.74 \\
    & SSIM $\uparrow$ & 0.8053 & 0.8078& 0.7572 & 0.7671& 0.7542 & 0.6576 & 0.7673 & 0.7691& 0.7073& 0.7515& 0.7835& \textcolor{red}{0.8422} \\
    & LPIPS $\downarrow$ & \textcolor{blue}{0.2847} & \textcolor{red}{0.2655} & 0.3169 & 0.3148& 0.3315 & 0.4599 & 0.4006 & 0.3189& 0.3760& 0.3665& 0.2968& 0.3381 \\
    & DISTS $\downarrow$ & \textcolor{blue}{0.2089} & \textcolor{red}{0.2055} & 0.2235 & 0.2219 & 0.2263 & 0.2749 & 0.2656 & 0.2315 & 0.2531 & 0.2485 & 0.2165 & 0.2524\\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_arc_lora}
\end{table*}

\noindent
\textbf{Layer-wise Importance.} Table \ref{table:effect_of_lora_layers} shows the impact of layer-specific updates for adapting SwinIR \cite{liang2021swinir} to real SR. Partitioning and evaluating convolutional layers reveals that certain layers, especially those in residual blocks (RSTLB Conv) and the final convolution layer after upsampling (AU Conv), achieve higher fidelity and perceptual scores with fewer parameter updates than MSA and MLP layers on DRealSR \cite{drealsr_wei2020component} at rank 32. Notably, the AU Conv layer delivers the highest performance gains, outperforming both the initial convolution layer (First Conv), the ones in the deep feature extraction module (DFE Convs) and pre-upsampling layer (BU Conv). Overall, adapting MLP linear layers or AU Conv optimally supports domain adaptation. 

% Analyzing individual LoRA layers highlights the role of layer-specific low-rank updates in adapting SwinIR \cite{liang2021swinir} to real SR. By partitioning the convolutional layers and evaluating each group, we provide a granular view of their effectiveness in domain adaptation. Table \ref{table:effect_of_lora_layers} shows that certain convolutional layers, particularly those in the residual blocks (RSTLB Conv) and final stages after upsampling (AU Conv), often yield higher fidelity and perceptual scores than the attention (MSA) and fully connected (MLP) layers, with fewer parameter updates on the DRealSR \cite{drealsr_wei2020component} dataset at rank 32. Specifically, adapting the final convolution layer (AU Conv) brings the largest performance gains with minimal parameter updates, outperforming the inital convolution layer (First Conv) and convolution layers before upsampling (BU Conv). Overall, adapting either MLP linear layers or the AU Conv in SwinIR best supports domain adaptation.

% \textcolor{red}{not understanding: this ablation needs to be modified after discussion. here u can also describe the method section that we discussed yesterday based on these layers. Then as we show in the ablation, the role of each indvidual component, we can show these layers role individually. what is sfe convolution , not wriiten in text. iF IT IS JUST FOR SWINIR, WE JUST HAD CONV LAYERS IN THE THREE PARTS AS U WROTE IN THE TEXT. }
 % Analyzing individual LoRA layers reveals the layer-wise importance of low-rank updates for effective adaptation to real SR for SwinIR \cite{liang2021swinir} architecture. As shown in Table \ref{table:effect_of_lora_layers}, MLP layers achieve the highest fidelity and perceptual scores on the DrealSR dataset at rank 32, with RSTLB convolution layers closely matching this performance while adapting 50$\%$ fewer parameters. RSTLB convolution layers are more efficient than MSA attention layers, as they provide better results with the less parameter updates. Furthermore, adapting the final convolution layer after upsampling (AU Conv) yields the greatest performance increase with minimal parameter updates, outperforming deep feature extraction (DFE) and before upsampling (BU) convolution layers. Overall, adapting either MLP linear layers or the AU Conv in SwinIR \cite{liang2021swinir} optimally supports domain adaptation. 

% Local attribution maps (LAM) \cite{lam_gu2021interpreting} are used to visualize the contribution of model components to feature interactions and contextual understanding. As shown in \ref{fig:saliency_image}, LAM demonstrates that combining LoRA layers enhances these interactions compared to individual sub-modules or full model fine-tuning. Diffusion index (DI) values show that LoRA applied to all layers achieves the widest attention range and best reconstruction performance, with convolution-only LoRA closely behind. Notably, even MLP-only LoRA outperforms standard fine-tuning. This analysis highlights that LoRA in all layers offers optimal adaptation with minimal parameter overhead (8$\%$ of trainable parameters), while focusing on convolution layers (2$\%$ parameters) is a lightweight yet effective alternative.

% We further extend our LoRA-based domain adaptation to GAN-based real-world SR, demonstrating versatility and efficiency. Using SwinIR \cite{liang2021swinir} as the baseline architecture with LoRA layers, we employ an adversarial training scheme with a U-Net discriminator with spectral normalization \cite{wang2021real}. For training,  we employ a weighted combination of L1, perceptual \cite{johnson2016perceptual}, and GAN losses (1:1:0.1) as in RealESRGAN. As shown in Table \ref{table:gan_result}, our method outperforms RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} in perceptual quality and fidelity while using only 886k parameters, compared to 12M in LDL and 17M in RealESRGAN. This highlights LoRA's ability to address complex real-world degradations with minimal computational overhead. This efficient, high-performing GAN-based domain adaptation approach further emphasizes the capability of LoRA to handle complex real-world degradations with reduced computational requirements.

%In addition to adapting bicubic-trained SR models, we extend our LoRA-based domain adaptation approach to GAN-based real-world SR, demonstrating its versatility and effectiveness. Using SwinIR \cite{liang2021swinir} as the baseline architecture with LoRA layers, we employ an adversarial training scheme with a U-Net discriminator with spectral normalization \cite{wang2021real}. For training, we apply a combination of L1 loss, perceptual loss \cite{johnson2016perceptual} and GAN loss with weightings of 1, 1, and 0.1, respectively, as in the RealESRGAN framework. Our approach achieves improved performance over existing GAN-based methods like RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} presented in Table \ref{table:gan_result} providing better perceptual quality and fidelity, while maintaining a significantly lower parameter count—only 886k trainable parameters compared to 12M in LDL and 17M in RealESRGAN. This efficient, high-performing GAN-based domain adaptation approach further emphasizes the capability of LoRA to handle complex real-world degradations with reduced computational requirements.

\subsection{Comparison with Other PEFT Methods}
\label{ss:comparison_peft}

\begin{table}
 \caption{PEFT methods vs. LoRA comparison on RealSR [4].} 
  \vspace{-0.3cm}
    \centering
    \scalebox{0.57}{
    \begin{tabular}{ccccccl}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{Model} & \multirow{2}{*}{PSNR} & \multirow{2}{*}{SSIM} & \multirow{2}{*}{LPIPS} & \multirow{2}{*}{DISTS} & Updated / Inference Time\\ 
    & & & & & Parameters \\
    \hline
    Baseline & 27.5537& 0.7738& 0.3965& 0.2426 & - / 12M \\
    FineTuning & 28.2637& 0.7922& 0.3016& 0.2274 & +12M / +12M \\
    ARC Adapter \cite{rebuttal_arc_dong2024efficient} (svd50) & 28.0836& 0.7894& 0.2995& 0.2206 & +125k / +125k \\
    ARC Adapter (svd100) & 28.0840& 0.7933& 0.2883& 0.2189 & +236k \ +236k \\
    ARC Adapter (svd350) & 28.2216& 0.7954& 0.2735& 0.2127 & +794k \ +794k\\
    ARC Adapter (svd375) & 28.3657& 0.7993& 0.2714& 0.2129 & +850k / +850k \\
    ARC Adapter (svd400) & 28.0856& 0.7924& 0.2760& 0.2144  & +906k / +906k \\ 
    ARC Adapter (svd500) & 28.1611& 0.7949& 0.2711& 0.2130 & +1.13M / +1.13M \\
    ARC Adapter (svd1000) & 28.4858& 0.7986& 0.2793& 0.2147 & +2.3M / +2.3M \\
    DiffFit PEFT & 28.2695& 0.7949& 0.2949& 0.2199& +13k / +13k \\
    AdaptSR (Ours) & 28.3999& 0.7976 & 0.2705& 0.2128 & +886k / -\\ 
    
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:adapter_vs_lora}
\vspace{-0.22cm}
\end{table}

\subsection{Generalization to Other Baselines}


\subsection{Comparison with State-of-the-Art}
\label{sec:comparison}
\textbf{Quantitative Performance.}
To comprehensively evaluate our LoRA-based domain adaptation approach, we applied it across diverse SR architectures: EDSR \cite{EDSR2017}, a simple yet efficient CNN model; SAFMN \cite{safmn_sun2023spatially}, a lightweight attention-based SR model; SwinIR \cite{liang2021swinir}, a transformer-based SR model; and DRCT \cite{drct_Hsu_2024_CVPR}, a high-capacity transformer for SR. This variety ensures comprehensive evaluation across both CNN and Transformer models. Table \ref{table:diff_arc_lora} presents the quantitative comparisons of our aforementioned LoRA-based SR methods and SoTA real GAN-based SR models (\textit{e.g.}, RealESRGAN \cite{wang2021real}, LDL \cite{liang2022details}) and diffusion models (e.g., PASD \cite{yang2023pasd}, SeeSR \cite{lora_diff_realsr_wu2024seesr}, OSEDiff \cite{lora_diff_realsr_wu2024one}) on $\times$4 real SR benchmarks. Compared to GAN-based methods like RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} which use over 20 times more parameters, our approach (e.g. SwinIR+LoRA) improves PSNR by up to 4 dB and perceptual scores (LPIPS) by 3$\%$ on RealSR \cite{realsr_cai2019toward} dataset while updating only 886k parameters. Similarly, diffusion models like SeeSR \cite{lora_diff_realsr_wu2024seesr} and PASD \cite{yang2023pasd}, with over 600 million parameters, as well as OSEDiff \cite{lora_diff_realsr_wu2024one} (8.5 million parameters, 10 times larger than our model), struggle to achieve competitive PSNR and SSIM performance. In contrast, SwinIR+LoRA outperforms OSEDiff by approximately 2 dB on DIV2K \cite{Agustsson_2017_CVPR_Workshops}, and by around 3.5 dB and 2.8 dB on the RealSR \cite{realsr_cai2019toward} and DRealSR \cite{drealsr_wei2020component} datasets, respectively. To conclude, our LoRA-based models excel in distortion metrics, achieving higher PSNR and SSIM across all datasets and demonstrating competitive LPIPS \cite{lpips} and DISTS \cite{dists} scores for perceptual quality with minimal parameter increases.

% Compared to GAN-based SR methods, which typically contain over 20 times more parameters, our LoRA-enhanced models achieve notable gains in performance. Specifically, our LoRA methods achieve up to a 3 dB improvement in PSNR and a 2$\%$ enhancement in perceptual scores (LPIPS) compared to GAN-based models, while updating only 8$\%$ of the parameters. Similarly, diffusion-based SR models containing over 100 million parameters exhibit lower performance, despite their extensive parameter count. Notably, OSEDiff \cite{lora_diff_realsr_wu2024one}, with 8.5 M parameters—over ten times larger than our LoRA-enhanced models—delivers significantly lower PSNR results. Specifically, our methods SwinIR+LoRA outperforms OSEDiff \cite{lora_diff_realsr_wu2024one} on DIV2K \cite{Agustsson_2017_CVPR_Workshops} by approximately 2 dB and on RealSR \cite{realsr_cai2019toward} and DRealSR \cite{drealsr_wei2020component} by about 3 dB. These results underscore the efficiency and adaptability of our LoRA-based approach, which achieves superior fidelity and perceptual quality with substantially fewer parameters than these heavier diffusion models.

\begin{table}
 \caption{\textit{Rank analysis} for better domain adaptation on RealSR \cite{realsr_cai2019toward} for 10k iterations. The best result is marked in \textbf{bold}.}
    \centering
    \scalebox{0.72}{
    \begin{tabular}{ccccccl}
    \specialrule{.1em}{.05em}{.05em} 
    Model & PSNR & SSIM & LPIPS & DISTS & Updated Paramaters\\  
    \hline
    Baseline & 27.5537& 0.7738& 0.3965& 0.2426 & 12M \\
    Baseline +FT & 28.2637& 0.7922& 0.3016& 0.2274 & +12M \\
    \hdashline
    r=1 &28.3383& 0.7957& 0.2772& 0.2129 &+152k (1.4\%)\\ 
    r=4 & 28.2675& 0.7945& 0.2721& \textbf{0.2125} & +466k (4.2\%)\\ 
    r=8 & \textbf{28.3999}& \textbf{0.7976}&\textbf{ 0.2705}& \textit{0.2128} & +886k (8.1\%)\\ 
    r=16 &\textit{28.3575}& \textit{0.7959}& 0.2719& 0.2140& +1.7M (15.5\%)\\ 
    r=64 & 28.3537& \textit{0.7959}& \textit{0.2716}& 0.2130 & +6.8M (61.8\%)\\ 
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular}  \vspace{-0.5cm}
}
\label{table:rank_analysis}
\end{table}

\begin{figure*}[t!]
\centering
\begin{subfigure}{0.285\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020hr_with_rectangle.pdf} \vspace{-8pt}\\ \centering \scriptsize DIV2K \cite{Agustsson_2017_CVPR_Workshops} \\ 807 (patch 00020)
    \end{subfigure}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031hr_with_rectangle.pdf} \vspace{-8pt}\\ \centering \scriptsize RealSR \cite{realsr_cai2019toward} \\ Nikon 31  
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.155\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020hr_crop.pdf} \vspace{-8pt}\\ \centering \scriptsize HR Crop \\ (PSNR / SSIM)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020osediff.pdf} \vspace{-8pt}\\ \centering \scriptsize OSEDiff \cite{lora_diff_realsr_wu2024one} \\ (11.559 / 0.772)
    \end{subfigure}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031hr_crop.pdf} \vspace{-8pt}\\ \centering \scriptsize HR Crop  \\ (PSNR / SSIM)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031osediff.pdf} \vspace{-8pt}\\ \centering \scriptsize OSEDiff \cite{lora_diff_realsr_wu2024one} \\ (19.801 / 0.943)
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.155\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020ldl_swinir.pdf}
        \vspace{-8pt}\\ \centering \scriptsize LDL \cite{liang2022details} \\ (9.627 / 0.727)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020safmn_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SAFMN+LoRA \\ (15.934 / 0.854)
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031ldl_swinir.pdf}
        \vspace{-8pt}\\ \centering \scriptsize LDL \cite{liang2022details} \\ (19.119 / 0.936)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031safmn_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SAFMN+LoRA \\ (25.738 / 0.976)    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.155\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020safmn.pdf} \vspace{-8pt}\\\centering \scriptsize  Real SAFMN-L \cite{safmn_sun2023spatially} \\ (10.686 / 0.760)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020swinir_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SwinIR + LoRA \\ (18.269 / 0.895)
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031safmn.pdf} \vspace{-8pt}\\\centering \scriptsize  Real SAFMN-L \cite{safmn_sun2023spatially} \\ (18.530 / 0.928)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031swinir_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SwinIR + LoRA \\ (29.463 / 0.987)
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.155\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020pasd.pdf} \vspace{-8pt}\\\centering \scriptsize PASD \cite{yang2023pasd} \\ (11.276 / 0.768)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020drct_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize DRCT + LoRA \\ (17.631 / 0.884)
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031pasd.pdf} \vspace{-8pt}\\\centering \scriptsize PASD \cite{yang2023pasd} \\ (21.608 / 0.953)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031drct_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize DRCT + LoRA \\ (28.729 / 0.986)
    \end{subfigure}
\end{subfigure}
\vspace{-3pt}
\caption{Visual comparison of the proposed LoRA-enhanced models with the state-of-the-art methods for $\times$4 real SR. GAN and diffusion models fail to capture the correct content of images, exhibit excessive sharpness with color shifts. On the other hand, our LoRA-based models reconstruct high-fidelity details with correct alignment, particularly in complex areas with regular patterns. Further visual comparisons, including fine-tuned model versions, are provided in the supplementary materials.}
\label{fig:qual_results} 
\end{figure*}

\noindent
\textbf{Qualitative Performance.} Figure \ref{fig:qual_results} illustrates visual comparisons among $\times$4 real SR methods, emphasizing the strengths of our LoRA-based domain-adapted approach. The qualitative results align closely with quantitative outcomes, revealing that GAN-SR models like LDL \cite{liang2022details} and Real SAFMN-Large \cite{safmn_sun2023spatially} show excessive sharpness with content inaccuracies such as misaligned striped patterns on roofs. Similarly, diffusion methods like PASD \cite{yang2023pasd} and OSEDiff \cite{lora_diff_realsr_wu2024one} introduce artifacts with inaccurate orientations for the first image. In contrast, our LoRA-based models successfully reconstruct fine details, accurately aligning roof stripes. Furthermore, in the second image, LDL \cite{liang2022details} and Real SAFM-L \cite{safmn_sun2023spatially} incorrectly render structure and colors. Likewise, diffusion methods PASD \cite{yang2023pasd} and OSEDiff \cite{lora_diff_realsr_wu2024one} produce inaccurate semantic generation. On the contrary, our LoRA-enhanced methods like SwinIR+LoRA and DRCT+LoRA preserve the correct structure and colors in the second case. Overall, our approach effectively controls artifacts while maintaining image fidelity, producing photorealistic, high-quality results in domain adaptation from bicubic to real SR.


% Figure \ref{fig:qual_results} illustrates visual comparisons among $\times$4 real SR approaches, highlighting the strengths of our LoRA-based domain adapted methods. Qualitative assessments closely align with the quantitative results, showing that GAN-SR models, including LDL \cite{liang2022details} and SAFMN-Large \cite{safmn_sun2023spatially}, often introduce artifacts, such as blending the man’s nose with the background or failing to reproduce textures. Similarly, diffusion-based methods like PASD \cite{yang2023pasd} and OSEDiff \cite{lora_diff_realsr_wu2024one} exhibit excessive sharpness with content inaccuracies, omitting details like the man’s mustache or failing to recover textures in the second patch. In contrast, our LoRA-based models adeptly reconstruct high-fidelity details, particularly in complex areas with regular patterns, such as retaining the man’s mustache and restoring textures in the second patch to match the HR image. Overall, our approach demonstrates a strong capacity to control artifacts while preserving accurate image details, achieving photorealistic, high-quality results in domain adaptation from bicubic to real SR.

\subsection{Ablation Study}
\label{sec:rank}
\noindent
\textbf{Rank Analysis.}
To identify the optimal LoRA rank for real SR adaptation, we conduct an ablation study by incrementally testing ranks from \( r = 1 \) to 64. Performance on the RealSR \cite{realsr_cai2019toward} dataset for $\times$4 images, shown in Table \ref{table:rank_analysis}, demonstrates that even at rank 1 (with only 1.4$\%$ of the trainable parameters), the results closely match those from fine-tuning with 12M parameters for SwinIR \cite{liang2021swinir}. Optimal fidelity for PSNR and SSIM and perceptual quality for LPIPS are achieved at \( r = 8 \). Higher ranks (16 and 64) do not yield additional gains but still outperform full fine-tuning with fewer parameter updates. These results align with prior findings of \cite{zeng2023expressive}, suggesting that larger models often require lower LoRA ranks for effective adaptation, especially when pre-trained models are well-suited to the target task. \textit{Rank analysis for other baselines and ablation studies for scaling factor are in supplementary materials.}

%This highlights LoRA’s efficiency in achieving efficient adaptation for even 1.4$\%$ parameter updates.

\begin{table}[t!]
 \caption{\textbf{Comparison of GAN-based RealSR }methods and our adversarially trained SwinIR$^G$ with LoRA method on DIV2K \cite{Agustsson_2017_CVPR_Workshops} validation patches. Our method achieves superior fidelity and perceptual quality with significantly fewer parameters.}
    \centering
    \scalebox{0.8}{
    \begin{tabular}{cccc}
    \specialrule{.1em}{.05em}{.05em} 
      & LDL (RealSwinIR) & RealESRGAN & SwinIR$^G$+LoRA \\ 
     % & 17M & 12M & 886k \\
     \hline
      Trainable & \multirow{2}{*}{17M} & \multirow{2}{*}{12M} & \multirow{2}{*}{886k}\\ 
      Parameters & & & \\
    \hline
    PSNR $\uparrow$ & 23.76 & 21.94 & \textbf{24.11}\\
    SSIM $\uparrow$ & 0.6403 & 0.5736 & \textbf{0.6598 }\\
    LPIPS $\downarrow$ & 0.3091 & 0.3868 & \textbf{0.2914 }\\
    DISTS $\downarrow$ & 0.2189 & 0.2601 &\textbf{ 0.2185}  \\ 
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:gan_result}
\end{table}

\noindent
\textbf{Extention to GAN-Based Real SR.} We further extend LoRA-based domain adaptation to GAN-based SR, showcasing its flexibility and efficiency. Using SwinIR \cite{liang2021swinir} with LoRA layers and a U-Net discriminator with spectral normalization \cite{wang2021real}, we apply adversarial training with a weighted combination of L1, perceptual \cite{johnson2016perceptual}, and GAN losses (1:1:0.1) as in RealESRGAN. As shown in Table \ref{table:gan_result}, our approach surpasses RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} in both fidelity and perceptual quality while using just 886k parameters, compared to 12M and 17M in LDL and RealESRGAN, respectively. These results highlight the effectiveness of LoRA-driven approach in enhancing GAN-based SR for real-world degradations, achieving fidelity results with minimal computational overhead.

% \section{Limitation and Future Work}
% Despite outperforming both GAN and diffusion methods with significantly smaller trainable parameters, our LoRA-based SR approach still faces limitations in fully capturing intricate textures and fine details. This challenge is common across existing SR methods, including ours, and highlights a need for more precise reconstruction of high-frequency components without increasing model size. Future work could address this by integrating multi-scale loss functions, texture-aware modules, or adaptive loss weighting based on regional texture complexity, refining fidelity and perceptual quality in challenging SR tasks.

% While our LoRA-based SR approach surpasses GAN- and diffusion-based methods with fewer parameters, it still encounters challenges in capturing intricate textures and fine details. This limitation shared across SR methods underscores the need for improved high-frequency reconstruction without increasing model size. Future work could address this by integrating multi-scale loss functions, texture-aware modules, or adaptive loss weighting based on regional texture complexity, refining fidelity and perceptual quality in challenging SR tasks.

==> sec/experiments_old.tex <==
\section{Experiments}
\subsection{Experimental Settings}
\noindent
\textbf{Datasets.}
We train all LoRA-enhanced networks on DIV2K \cite{Agustsson_2017_CVPR_Workshops} and RealSR \cite{realsr_cai2019toward} training sets, using the Real-ESRGAN \cite{wang2021real} degradation pipeline to create LR-HR pairs. During training, we also utilize the DIV2K unknown degradation dataset to cover a wider range of degradation types, using randomly cropped $256\times256$ patches from the HR images. For evaluation, we benchmark against other methods on DIV2K, RealSR, and DRealSR \cite{drealsr_wei2020component} test sets. It is to be noted that to compare with diffusion-based approaches, we adopt the StableSR \cite{wang2024exploiting} validation setup, including 3000 patches from DIV2K, 100 from RealSR, and 93 from DRealSR, with LR-HR pairs sized at $128\times128$ and $512\times512$.

\noindent
\textbf{Implementation Details and Evaluation.}
All experiments were run on an NVIDIA Quadro RTX 4090 GPU using PyTorch. LoRA models were trained for 100k iterations with Adam \cite{kingma2014adam} and L1 loss, starting with a learning rate of $1e^{-3}$, reduced by 25$\%$ at 50k, 75k, and 90k iterations. In comparison, full model fine-tuning on a Tesla V100 GPU required 500k iterations, with the learning rate halved at specific intervals. Both LoRA and fine-tuning used the same settings, including the Adam optimizer \cite{kingma2014adam}, a batch size of 8, and the L1 loss function. To evaluate fidelity and perceptual quality, we used PSNR and SSIM (Y channel in YCbCr space) and perceptual metrics LPIPS \cite{lpips} and DISTS \cite{dists}.


% All experiments were conducted on an NVIDIA Quadro RTX 4090 GPU using the PyTorch framework. We trained all LoRA models for 100k iterations with the Adam optimizer \cite{kingma2014adam} and L1 loss function, using a mini-batch size of 8 and an initial learning rate of $1e^{-3}$. The learning rate was decreased by 25$\%$ at the 50k, 75k, and 90k iterations. In contrast, full model fine-tuning on Tesla V100 GPU required 500k iterations with the learning rate halved at 250k, 400k, 450k and 475k iterations. For finetuning experiments, we used the same settings as for the LoRA models; an initial learning rate of $1e^{-3}$, a mini-batch size of 8, and the Adam optimizer \cite{kingma2014adam} with the L1 loss function.

% To comprehensively assess the performance of our LoRA methods and other state-of-the-art GAN-based and diffusion-based real SR methods, we use both full-reference and no-reference metrics. PSNR and SSIM (computed on the Y channel in YCbCr space) serve as fidelity metrics with ground-truth reference, while LPIPS \cite{lpips} and DISTS \cite{dists} measure perceptual quality. For no-reference quality assessment, we employ NIQE \cite{niqe_zhang2015feature}, MUSIQ \cite{ke2021musiq}, MANIQA \cite{yang2022maniqa} and CLIPIQA \cite{clipiqa_wang2022exploring}.

\subsection{Adapting LoRA Layers vs. Fine-Tuning}
\label{sec:fine}
Table \ref{table:diff_degredation_lora} presents a comparison between LoRA-based adaptation and standard fine-tuning for $\times$4 real super-resolution on SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially} using the RealSR validation set\cite{realsr_cai2019toward}. 
It is clear that LoRA delivers similar or better performance than fine-tuning with significantly less memory and computational cost. For SwinIR \cite{liang2021swinir}, LoRA boosts PSNR by 0.42 dB, SSIM by 2$\%$, and LPIPS by 3.2$\%$ while updating only 886k parameters versus 12M for fine-tuning. For lightweight SAFMN \cite{safmn_sun2023spatially}, LoRA achieves similar gains with just around 100k parameters which is half of the parameters required for fine-tuning. Crucially, since LoRA layers are merged into the base model post-training, inference speed remains unchanged. Furthermore, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA converges within 100k iterations, taking 5 hours on SwinIR and 2.5 hours on SAFMN on an NVIDIA RTX 4090, compared to 4 days and 1 day, respectively, for fine-tuning. These results highlight efficiency and high performance of LoRA adaptation as a fine-tuning alternative, offering strong fidelity and perceptual quality with minimal training time.

\begin{figure}
\centering
\input{images/training_time_vs_psnr_ft_vs_lora}
\caption{Number of iterations vs. performance comparison for full model finetuning and LoRA-enhanced models for SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially}. LoRA reaches peak PSNR in just 100k iterations, completing in 5 hours for SwinIR and 2.5 hours for SAFMN on an NVIDIA RTX 4090, whereas fine-tuning takes significantly longer—4 days for SwinIR and 1 day for SAFMN—to achieve similar performance. The dashed lines of LoRA methods indicate their final PSNR performance at their latest iteration 100k.}
\label{fig:numiter_vs_psnr}
\end{figure}

\begin{table}
 \caption{\textbf{Performance comparison for domain adaptation between fine-tuning and LoRA-enhanced models} on RealSR \cite{realsr_cai2019toward}. LoRA matches or outperforms standard fine-tuning on SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially} models with significantly fewer trainable parameters and shorter training time, while maintaining the inference speed of baseline models. Here, $^{*}$ denotes the bi-cubically trained model.}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{cccccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{Model} & \multirow{2}{*}{PSNR} & \multirow{2}{*}{SSIM} & \multirow{2}{*}{LPIPS} & Trainable & GPU\\
     & & &  & Parameters & Hours \\  
    \hline
    SwinIR$^{*}$ & 27.5537 & 0.7738 & 0.3965 & 12M & -\\
     + FineTuning & 28.2537 & 0.7906 & 0.3820 & +12M & 96 \\
     + LoRA & 28.6964 & 0.8079 & 0.2591 & +886k & 5 \\ 
     \hdashline
    SAFMN$^{*}$  & 27.5383 & 0.7740 & 0.3927 & 240k & -\\
     + FineTuning & 28.3173 & 0.7936 & 0.2887 & +240k & 28 \\
     + LoRA & 28.3245 & 0.7935 & 0.2935 & +99.5k & 2.5 \\ 
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_degredation_lora}
\end{table}

% Table \ref{table:diff_degredation_lora} compares LoRA-based adaptation with standard fine-tuning for $\times$4 SR on Transformer-based SwinIR \cite{liang2021swinir} and CNN-based SAFMN \cite{safmn_sun2023spatially}, evaluated on the DIV2K unknown validation set \cite{Agustsson_2017_CVPR_Workshops}. LoRA delivers comparable or superior performance to fine-tuning while significantly reducing memory and computational demands. For SwinIR, LoRA improves PSNR by 0.75 dB, SSIM by $2.5\%$, and LPIPS by $5.8\%$ while updating only 886k parameters ($8\%$ of total) compared to 12M for fine-tuning. For SAFMN, LoRA achieves similar results with only 100k updated parameters—half the amount required by fine-tuning. Crucially, since LoRA layers are merged into the base model post-training, inference speed remains unchanged. Furthermore, as shown in Figure \ref{fig:numiter_vs_psnr}, LoRA converges within 100k iterations, requiring just 5 hours for SwinIR and 2.5 hours for SAFMN on an NVIDIA RTX 4090, compared to 4 days and 1 day for fine-tuning, respectively. These results highlight LoRA adapted approaches as a memory-efficient, high-performance alternative to fine-tuning, providing strong fidelity and perceptual quality with minimal training overhead.
%Table \ref{table:diff_degredation_lora} compares LoRA-based adaptation with standard fine-tuning on the $\times$4 SR task using SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially} models, evaluated on the DIV2K unknown validation set \cite{Agustsson_2017_CVPR_Workshops}. LoRA achieves comparable or superior results to fine-tuning while greatly reducing memory and computational costs for both baseline models. Specifically, for SwinIR \cite{liang2021swinir}, LoRA surpasses fine-tuning by 0.75 dB in PSNR, $2.5\%$ in SSIM, and $5.8\%$in LPIPS, while updating only 886k parameters ($8\%$ of all parameters) compared to 12M for fine-tuning. For the lightweight SAFMN \cite{safmn_sun2023spatially} model, LoRA achieves comparable performance to fine-tuning while updating only 100k parameters—half the number required by fine-tuning. Importantly, since LoRA layers are merged into the base model after training, inference speed remains the same as the original model. As shown in Figure \ref{fig:numiter_vs_psnr}, LoRA reaches peak PSNR within 100k iterations, requiring only 5 hours and 2.5 hours on an NVIDIA RTX 4090, for SwinIR and SAFMN, respectively. On the other hand, fine-tuning SwinIR takes 4 days and SAFMN requires 1 day to achieve comparable performance. These results confirm that LoRA is a high-performance, memory-efficient alternative to fine-tuning, offering strong fidelity and perceptual quality with minimal training overhead.

% \begin{figure}
% \centering
% \includegraphics[width=\linewidth]{images/training_time_vs_psnr_ft_vs_lora}
% \caption{Number of iterations vs. performance comparison for full model finetuning and LoRA-enhanced models for SwinIR \cite{liang2021swinir} and SAFMN \cite{safmn_sun2023spatially}. LoRA reaches peak PSNR in just 100k iterations, completing in 5 hours for SwinIR and 2.5 hours for SAFMN on an NVIDIA RTX 4090, whereas fine-tuning takes significantly longer—4 days for SwinIR and 1 day for SAFMN—to achieve similar performance.}
% \label{fig:numiter_vs_psnr}
% \end{figure}



% \begin{table*}
%  \caption{Performance comparison of SR models for domain adaptation from bicubic to real SR. LoRA-enhanced models consistently improve fidelity and perceptual quality over baseline methods with minimal additional parameters.}
%     \centering
%     \scalebox{0.9}{
%     \begin{tabular}{ccccccccc}
%     \specialrule{.1em}{.05em}{.05em} 
%      Metric & EDSR & EDSR+LoRA & SAFMN & SAFMN+LoRA & SwinIR & SwinIR+LoRA & DRCT & DRCT+LoRA \\ 
%      & & +300k & & +99.5k & & +886k & & +3M \\
%      \hline
%      PSNR $\uparrow$ & 27.5422& 27.9260& 27.5583& 28.3245& 27.5537& 28.6964& 27.5502& 28.7173\\
%      SSIM $\uparrow$ &  0.7732 & 0.7878 & 0.7740 & 0.7935 & 0.7738 & 0.8079 & 0.7737 & 0.8061 \\
%      LPIPS $\downarrow$ &  0.3937&0.2835&0.3927&0.2935&0.3965&0.2591&0.3966&0.2553 \\
%      DISTS $\downarrow$ &  0.2436&0.2190&0.2430&0.2229&0.2426&0.2109&0.2434&0.2094 \\ 
%      % CLIPIQA$\uparrow$& 0.3289&0.2829&0.3338&0.2614&0.3388&0.3264&0.3384&0.3206\\
%      % NIQE$\downarrow$ &  8.3179&7.8546&8.3443&7.7209&8.3294&8.3661&8.3130&8.3144 \\
%      % MUSIQ$\uparrow$ & 30.8765&43.9013&30.7043&41.8672&30.5589&48.4967&30.5884&48.0846 \\
%      %  MANIQA $\uparrow$ &  0.3642 & 0.3766 & 0.3703 & 0.3780 & 0.3711 & 0.3947 & 0.3671 & 0.3968 \\
% \specialrule{.1em}{.05em}{.05em} 
%     \end{tabular} 
% }
% \label{table:domain_adaptation}
% \end{table*}

\subsection{Bicubic to Real SR with LoRA}
Table \ref{table:domain_adaptation} summarizes the performance of SoTA CNN and Transformer-based SR models adapted from bicubic to real-world SR using LoRA layers. Across models including EDSR \cite{EDSR2017}, SAFMN \cite{safmn_sun2023spatially}, SwinIR \cite{liang2021swinir}, and DRCT \cite{drct_Hsu_2024_CVPR}, LoRA adaptation significantly enhances both fidelity and perceptual quality. LoRA models achieve up to a 1 dB PSNR boost and a 4$\%$ SSIM increase for all models compared to their bicubic baselines. Specifically, SwinIR+LoRA notably gains 1.14 dB in PSNR and 4.4$\%$ in SSIM over bicubic-trained models on the RealSR \cite{realsr_cai2019toward} dataset. Perceptual metrics like LPIPS \cite{lpips} and DISTS \cite{dists} also indicate reduced artifacts and improved visual quality, as detailed in Sec. \ref{sec:qual}. This demonstrates the effectiveness of LoRA in achieving efficient domain adaptation for real-world SR neither requiring long hours of GPU training nor sacrificing the inference speed and perceptual quality.

\begin{table}
 \caption{\textbf{Performance comparison of LoRA-enhanced models for domain adaptation} from bicubic to real SR. LoRA-enhanced models consistently improve fidelity and perceptual quality over baseline methods with minimal additional parameters on RealSR \cite{realsr_cai2019toward} dataset.}
    \centering
    \scalebox{0.85}{
    \begin{tabular}{cccccc}
    \specialrule{.1em}{.05em}{.05em} 
     Method & Params &PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & DISTS $\downarrow$ \\
     \hline
     EDSR & & 27.5422 & 0.7732 & 0.3937 & 0.2436 \\
     +FineTuning & & 28.1605& 0.7963& 0.2703& 0.2179 \\
     + LoRA & +300k &27.9260 & 0.7878 & 0.2835 & 0.2190 \\
     SAFMN & &27.5583 & 0.7740 & 0.3927 & 0.2430 \\
     +LoRA & +99.5k &28.3245 & 0.7935 & 0.2935 & 0.2229 \\
     SwinIR & &27.5537 & 0.7738 & 0.3965 & 0.2426 \\
     + LoRA & +886k &28.6964 & 0.8079 & 0.2591 & 0.2109 \\
     DRCT & &27.5502 & 0.7737 & 0.3966 & 0.2434 \\ 
     + FineTuning & & 28.7481& 0.8100& 0.2467& 0.2086 \\
     + LoRA & +3M &28.7173 & 0.8061 & 0.2553 & 0.2094 \\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:domain_adaptation}
\end{table}
 
%Table \ref{table:domain_adaptation} presents the performance of various SR models adapted from bicubic training to real-world SR using LoRA layers. Across all tested models; EDSR \cite{EDSR2017}, SAFMN \cite{safmn_sun2023spatially}, SwinIR \cite{liang2021swinir} and DRCT \cite{drct_Hsu_2024_CVPR}, training LoRA layers for domain adaptation significantly boosts both fidelity and perceptual quality. In terms of PSNR and SSIM, LoRA-enhanced models consistently outperform their baseline counterparts, with improvements of up to 1 dB in PSNR and noticeable gains of 4$\%$ in SSIM. For instance, SwinIR+LoRA improves baseline PSNR performance by 1.14 dB and SSIM performance by 4.4$\%$. Moreover, these improvements extend to perceptual metrics as well. LoRA-enhanced models exhibit lower LPIPS \cite{lpips} and DISTS \cite{dists} scores, indicating a reduction in perceptual artifacts and an overall improvement in visual quality. Importantly, since LoRA layers are merged with the base model after training, the inference time remains identical to the baseline while maintaining computational efficiency. This demonstrates the effectiveness of LoRA in achieving efficient domain adaptation for real-world SR neither requiring long hours of GPU training nor sacrificing the inference speed.

\subsection{Module-wise Importance for Adaptation}
\label{sec:adapt}
% To determine the most critical modules for domain adaptation from bicubic to real SR, we applied LoRA to specific components in SwinIR \cite{liang2021swinir} in four configurations: (1) all layers (convolutional, linear, and attention layers), (2) only convolutional layers, (3) only multi-head self-attention (MSA) layers, and (4) only MLP layers. Figure \ref{fig:training_time_vs_psnr} compares training time and PSNR for these configurations over 10k iterations. Applying LoRA across all layers achieved full fine-tuning performance in just 50 minutes (vs. 4 days), with only 8$\%$ of parameters. LoRA applied to convolutional layers alone, with just 2$\%$ of parameters, reached near full-tuning performance within 30 minutes. Notably, LoRA models began at a PSNR of 22.606 dB, matching the bicubic baseline's initial performance. 
To identify the most crucial modules for adapting SwinIR \cite{liang2021swinir} from bicubic to real SR, we tested LoRA on four configurations: (1) all layers (convolutional, linear, and attention), (2) only convolutional layers, (3) only multi-head self-attention (MSA) layers, and (4) only MLP layers. As illustrated in Figure \ref{fig:training_time_vs_psnr}, applying LoRA to all layers achieved full fine-tuning results in just 50 minutes (compared to 4 days), using only 8$\%$ of the original parameters. Focusing solely on convolutional layers achieved comparable performance within 30 minutes with only 2$\%$ of parameters. Notably, all configurations began at 22.606 dB PSNR, matching the initial bicubic baseline.

% Local attribution maps (LAM) \cite{lam_gu2021interpreting} are used to visualize the contribution of model components to feature interactions and contextual understanding. As shown in Figure \ref{fig:saliency_image}, LAM demonstrates that combining LoRA layers enhances these interactions compared to individual sub-modules or full model fine-tuning. 

Local Attribution Maps (LAM) \cite{lam_gu2021interpreting} visualize the contributions of components to feature interactions and context. Figure \ref{fig:saliency_image} shows that combining LoRA layers enhances these interactions beyond individual modules or full fine-tuning.Diffusion index (DI) \cite{lam_gu2021interpreting} values, indicating attention range, confirm that LoRA applied to all layers achieves the widest attention and strongest reconstruction and it is followed closely by the convolution-only LoRA performance. Remarkably, MLP-only LoRA still surpasses standard fine-tuning in feature capture. This module analysis shows that LoRA in all layers is optimal for adaptation, with minimal parameter overhead, while focusing solely on convolutional layers (2$\%$ parameters) offers a highly efficient alternative. \textit{Additional module-wise analysis for other architectures are included in the supplementary.}

\begin{figure}
    \centering
    \input{images/training_time_vs_psnr_for_lora_modules.tex}
\caption{Training time vs. performance comparison for different LoRA modules with 10k iterations. The dashed line indicates the best PSNR achieved by standard fine-tuning, which requires 4 days of training. Notably, LoRA applied to all layers reaches this PSNR level in just 30 minutes.}
\label{fig:training_time_vs_psnr}
\end{figure}

\begin{table}
 \caption{\textbf{Layer-wise importance for LoRA domain adaptation} from bicubic to real SR on DRealSR \cite{drealsr_wei2020component} dataset.}
    \centering
    \scalebox{0.75}{
    \begin{tabular}{cccccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{LoRA Layer} & \multirow{2}{*}{PSNR} & \multirow{2}{*}{SSIM} & \multirow{2}{*}{LPIPS} & Trainable &  Training \\
    & & & & Parameters & Time (Mins)\\ 
    \hline
   All Convs & 30.9736 & 0.8425 & 0.3994 & 868k & 31.45 \\
   MSAs  & 30.7712 & 0.8402 & 0.4023 & 1.2M & 77 \\
   MLPs  & 31.0241 & 0.8433 & 0.3999 & 1.2M & 57.71 \\
   \hdashline
   First Conv & 30.0777 & 0.8226 & 0.4327 & 53k & 24.95 \\
   RSTLB Convs & 30.9682 & 0.8422 & 0.4003 & 622k & 41.09 \\
   DFE Convs & 29.5300 & 0.8088 & 0.4470 & 104k & 19.22 \\
   BU Conv & 29.5828 & 0.8117 & 0.4379 & 70k & 19.02  \\
   AU Conv & 30.4789 & 0.8305 & 0.4201 & 19k & 18.42 \\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:effect_of_lora_layers}
\end{table}

\begin{figure}
\centering
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/position_pil_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{Nikon 41 \\ DI \cite{lam_gu2021interpreting}}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/fine-tuned_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{SwinIR \cite{liang2021swinir} FT \\  16.08}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_attn_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
    \caption*{Attention Blocks \\ 14.72}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_mlp_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{MLP Blocks \\ 17.27}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/lora_all_convs_only_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{Conv Layers \\ 18.78}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{images/all_lora_saliency_image_abs_Nikon_041_HR_104.png} 
    \end{subfigure}
\caption*{All Layers \\ 19.59}
\end{subfigure}
\caption{Comparison of \textbf{local attribution maps} (LAMs) \cite{lam_gu2021interpreting} between different LoRA modules and standard fine-tuning model on RealSR-Nikon41  \cite{realsr_cai2019toward} image. The LAM results denote the importance of each pixel in the input image when super-resolving the patch marked with a red box. The diffusion index (DI) \cite{lam_gu2021interpreting} value reflects the range of involved pixels hence better reconstruction.} \vspace{-0.5cm}
\label{fig:saliency_image} 
\end{figure} 

\begin{table*}[t!]
 \caption{Quantitative comparison of the proposed Low-Rank adaptation from bicubic domain to real SR methods representing the generalization capability of domain adaptation of LoRA SR. The best and the second-best results of each metric are highlighted in \textcolor{red}{red} and \textcolor{blue}{blue}, respectively.
 }
    \centering
    \scalebox{0.7}{
    \begin{tabular}{c|l|ccc|cccc|cccc}
    \specialrule{.1em}{.05em}{.05em} 
    & & \multicolumn{3}{|c|}{GAN-based Real SR} & \multicolumn{4}{c|}{Diffusion-based Real SR} & \multicolumn{4}{c}{Ours} \\
    \hline
    & & RealESRGAN & LDL & Real-SAFMN-L & SeeSR & PASD & SinSR & OSEDiff & EDSR+LoRA & SAFMN+LoRA & SwinIR+LoRA & DRCT+LoRA \\
    \hline
     \multirow{2}{*}{\centering Dataset} & Trainable & \multirow{2}{*}{\centering 17M} & \multirow{2}{*}{\centering 12M} & \multirow{2}{*}{\centering 5.6M}& \multirow{2}{*}{\centering 750M} & \multirow{2}{*}{\centering 625M} & \multirow{2}{*}{\centering 119M}& \multirow{2}{*}{\centering 8.5M}& \multirow{2}{*}{\centering 314k} & \multirow{2}{*}{\centering 99.5k}& \multirow{2}{*}{\centering 886k} & \multirow{2}{*}{\centering 3.1M} \\
    & Parameters & & & & & & & & & & & \\
    \hline
    \multirow{4}{*}{\centering DIV2K} & PSNR $\uparrow$ & 22.94 & 23.76 & 23.21 & 23.68 & 23.14 & 24.41 & 23.72 & 25.54 & 25.47 & \textcolor{red}{25.81} & \textcolor{blue}{25.77} \\
    & SSIM $\uparrow$ &  0.6036 &  0.6403&  0.5950&  0.6043 &  0.5505 &  0.6018 &  0.6108 &  0.6553&  0.6547&  \textcolor{blue}{0.6681} &  \textcolor{red}{0.6693} \\
    & LPIPS $\downarrow$ &  0.3768 & \textcolor{blue}{0.3091}&  0.3282&  0.3194 &  0.3571 &  0.3240 &  \textcolor{red}{0.2941} &  0.5376&  0.5461&  0.5047&  0.5037 \\
    & DISTS $\downarrow$ &  0.2520&  0.2189&  0.2153&  \textcolor{red}{0.1968}&  0.2207&  0.2066&  \textcolor{blue}{0.1976}&  0.3324&  0.3271&  0.3194&  0.3167 \\
    \hline
    \multirow{4}{*}{\centering RealSR} & PSNR $\uparrow$ & 25.69 & 24.96 & 24.23 & 25.18 & 25.21 & 26.28 & 25.15 & 27.93 & 28.32 & \textcolor{blue}{28.70} & \textcolor{red}{28.72} \\
    & SSIM $\uparrow$ &  0.7616 &  0.7634&  0.7217&  0.7216&  0.6798&  0.7347&  0.7341&  0.7878&  0.7935&  \textcolor{red}{0.8079} &  \textcolor{blue}{0.8061} \\
    & LPIPS $\downarrow$ &  0.2727 & \textcolor{red}{0.2519}&  0.2905&  0.3009&  0.3380&  0.3188&  0.2921&  0.2835&  0.2935&  0.2591&  \textcolor{blue}{0.2553} \\
    & DISTS $\downarrow$ &  \textcolor{blue}{0.2063}& \textcolor{red}{0.1981}&  0.2176&  0.2223&  0.2260&  0.2353&  0.2128&  0.2190&  0.2229&  0.2109&  0.2094 \\
     \hline
    \multirow{4}{*}{\centering DRealSR} & PSNR $\uparrow$ & 28.64 & 27.43 & 27.15 & 28.17 & 27.36 & 28.36 & 27.92 & 30.64 & \textcolor{red}{30.92} & 30.74 & \textcolor{blue}{30.81} \\
    & SSIM $\uparrow$ & 0.8053 & 0.8078& 0.7671& 0.7691& 0.7073& 0.7515& 0.7835& 0.8368& 0.8403& \textcolor{red}{0.8422}& \textcolor{blue}{0.8419} \\
    & LPIPS $\downarrow$ & \textcolor{blue}{0.2847} & \textcolor{red}{0.2655} & 0.3148& 0.3189& 0.3760& 0.3665& 0.2968& 0.3523& 0.3529& 0.3381& 0.3414 \\
    & DISTS $\downarrow$ & \textcolor{blue}{0.2089} & \textcolor{red}{0.2055} & 0.2219 & 0.2315 & 0.2531 & 0.2485 & 0.2165 & 0.2548 & 0.2545 & 0.2524 & 0.2544\\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_arc_lora}
\end{table*}

\noindent
\textbf{Layer-Wise Importance.} Table \ref{table:effect_of_lora_layers} shows the impact of layer-specific updates for adapting SwinIR \cite{liang2021swinir} to real SR. Partitioning and evaluating convolutional layers reveals that certain layers, especially those in residual blocks (RSTLB Conv) and the final convolution layer after upsampling (AU Conv), achieve higher fidelity and perceptual scores with fewer parameter updates than MSA and MLP layers on DRealSR \cite{drealsr_wei2020component} at rank 32. Notably, the AU Conv layer yields the largest performance gains, surpassing initial (First Conv) and pre-upsampling (BU Conv) layers. Overall, adapting MLP linear layers or AU Conv optimally supports domain adaptation. 

% Analyzing individual LoRA layers highlights the role of layer-specific low-rank updates in adapting SwinIR \cite{liang2021swinir} to real SR. By partitioning the convolutional layers and evaluating each group, we provide a granular view of their effectiveness in domain adaptation. Table \ref{table:effect_of_lora_layers} shows that certain convolutional layers, particularly those in the residual blocks (RSTLB Conv) and final stages after upsampling (AU Conv), often yield higher fidelity and perceptual scores than the attention (MSA) and fully connected (MLP) layers, with fewer parameter updates on the DRealSR \cite{drealsr_wei2020component} dataset at rank 32. Specifically, adapting the final convolution layer (AU Conv) brings the largest performance gains with minimal parameter updates, outperforming the inital convolution layer (First Conv) and convolution layers before upsampling (BU Conv). Overall, adapting either MLP linear layers or the AU Conv in SwinIR best supports domain adaptation.

% \textcolor{red}{not understanding: this ablation needs to be modified after discussion. here u can also describe the method section that we discussed yesterday based on these layers. Then as we show in the ablation, the role of each indvidual component, we can show these layers role individually. what is sfe convolution , not wriiten in text. iF IT IS JUST FOR SWINIR, WE JUST HAD CONV LAYERS IN THE THREE PARTS AS U WROTE IN THE TEXT. }
 % Analyzing individual LoRA layers reveals the layer-wise importance of low-rank updates for effective adaptation to real SR for SwinIR \cite{liang2021swinir} architecture. As shown in Table \ref{table:effect_of_lora_layers}, MLP layers achieve the highest fidelity and perceptual scores on the DrealSR dataset at rank 32, with RSTLB convolution layers closely matching this performance while adapting 50$\%$ fewer parameters. RSTLB convolution layers are more efficient than MSA attention layers, as they provide better results with the less parameter updates. Furthermore, adapting the final convolution layer after upsampling (AU Conv) yields the greatest performance increase with minimal parameter updates, outperforming deep feature extraction (DFE) and before upsampling (BU) convolution layers. Overall, adapting either MLP linear layers or the AU Conv in SwinIR \cite{liang2021swinir} optimally supports domain adaptation. 

% Local attribution maps (LAM) \cite{lam_gu2021interpreting} are used to visualize the contribution of model components to feature interactions and contextual understanding. As shown in \ref{fig:saliency_image}, LAM demonstrates that combining LoRA layers enhances these interactions compared to individual sub-modules or full model fine-tuning. Diffusion index (DI) values show that LoRA applied to all layers achieves the widest attention range and best reconstruction performance, with convolution-only LoRA closely behind. Notably, even MLP-only LoRA outperforms standard fine-tuning. This analysis highlights that LoRA in all layers offers optimal adaptation with minimal parameter overhead (8$\%$ of trainable parameters), while focusing on convolution layers (2$\%$ parameters) is a lightweight yet effective alternative.

% We further extend our LoRA-based domain adaptation to GAN-based real-world SR, demonstrating versatility and efficiency. Using SwinIR \cite{liang2021swinir} as the baseline architecture with LoRA layers, we employ an adversarial training scheme with a U-Net discriminator with spectral normalization \cite{wang2021real}. For training,  we employ a weighted combination of L1, perceptual \cite{johnson2016perceptual}, and GAN losses (1:1:0.1) as in RealESRGAN. As shown in Table \ref{table:gan_result}, our method outperforms RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} in perceptual quality and fidelity while using only 886k parameters, compared to 12M in LDL and 17M in RealESRGAN. This highlights LoRA's ability to address complex real-world degradations with minimal computational overhead. This efficient, high-performing GAN-based domain adaptation approach further emphasizes the capability of LoRA to handle complex real-world degradations with reduced computational requirements.

%In addition to adapting bicubic-trained SR models, we extend our LoRA-based domain adaptation approach to GAN-based real-world SR, demonstrating its versatility and effectiveness. Using SwinIR \cite{liang2021swinir} as the baseline architecture with LoRA layers, we employ an adversarial training scheme with a U-Net discriminator with spectral normalization \cite{wang2021real}. For training, we apply a combination of L1 loss, perceptual loss \cite{johnson2016perceptual} and GAN loss with weightings of 1, 1, and 0.1, respectively, as in the RealESRGAN framework. Our approach achieves improved performance over existing GAN-based methods like RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} presented in Table \ref{table:gan_result} providing better perceptual quality and fidelity, while maintaining a significantly lower parameter count—only 886k trainable parameters compared to 12M in LDL and 17M in RealESRGAN. This efficient, high-performing GAN-based domain adaptation approach further emphasizes the capability of LoRA to handle complex real-world degradations with reduced computational requirements.

\subsection{Comparison with State-of-the-Art}
\textbf{Quantitative Performance.}
% \textcolor{red}{too long will rephrase once tables are finaliseed }
To comprehensively evaluate our LoRA-based domain adaptation approach, we applied it across diverse SR architectures: EDSR \cite{EDSR2017}, a simple yet efficient CNN model; SAFMN \cite{safmn_sun2023spatially}, a lightweight attention-based SR model; SwinIR \cite{liang2021swinir}, a transformer-based SR model; and DRCT \cite{drct_Hsu_2024_CVPR}, a high-capacity transformer for SR. This variety ensures comprehensive evaluation across both CNN and transformer models.

% To comprehensively evaluate our LoRA-based domain adaptation approach, we applied it across a variety of SR architectures including EDSR \cite{EDSR2017}, a simple yet efficient convolutional model; SAFMN \cite{safmn_sun2023spatially}, a lightweight SR model with attention mechanism; SwinIR \cite{liang2021swinir}, a transformer-based SR model; and DRCT \cite{drct_Hsu_2024_CVPR}, a heavy transformer model for high-capacity SR tasks. This diversity ensures a comprehensive evaluation across CNN and transformer-based models.

Table \ref{table:diff_arc_lora} presents the quantitative comparisons of our aforementioned LoRA-based SR methods and state-of-the-art real GAN-based SR models (\textit{e.g.}, RealESRGAN \cite{wang2021real}, LDL \cite{liang2022details}) and diffusion models (e.g., PASD \cite{yang2023pasd}, SeeSR \cite{lora_diff_realsr_wu2024seesr}, OSEDiff \cite{lora_diff_realsr_wu2024one}) on $\times$4 real benchmark SR datasets. Compared to GAN-based methods like RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} which use over 20 times more parameters, our approach (e.g. SwinIR+LoRA) improves PSNR by up to 4 dB and perceptual scores (LPIPS) by 3$\%$ on RealSR \cite{realsr_cai2019toward} dataset while updating only 886k parameters. 
Similarly, diffusion models like SeeSR \cite{lora_diff_realsr_wu2024seesr} and PASD \cite{yang2023pasd}, with over 600 million parameters, as well as OSEDiff \cite{lora_diff_realsr_wu2024one} (8.5 million parameters, more than 10 times larger than our model), struggle to achieve competitive PSNR and SSIM performance. In contrast, SwinIR+LoRA outperforms OSEDiff by approximately 2 dB on DIV2K \cite{Agustsson_2017_CVPR_Workshops}, and by around 3.5 dB and 2.8 dB on the RealSR \cite{realsr_cai2019toward} and DRealSR \cite{drealsr_wei2020component} datasets, respectively. To conclude, our LoRA-based models excel in distortion metrics, achieving higher PSNR and SSIM across all datasets and demonstrating competitive LPIPS \cite{lpips} and DISTS \cite{dists} scores for perceptual quality with minimal parameter increases.

% Compared to GAN-based SR methods, which typically contain over 20 times more parameters, our LoRA-enhanced models achieve notable gains in performance. Specifically, our LoRA methods achieve up to a 3 dB improvement in PSNR and a 2$\%$ enhancement in perceptual scores (LPIPS) compared to GAN-based models, while updating only 8$\%$ of the parameters. Similarly, diffusion-based SR models containing over 100 million parameters exhibit lower performance, despite their extensive parameter count. Notably, OSEDiff \cite{lora_diff_realsr_wu2024one}, with 8.5 M parameters—over ten times larger than our LoRA-enhanced models—delivers significantly lower PSNR results. Specifically, our methods SwinIR+LoRA outperforms OSEDiff \cite{lora_diff_realsr_wu2024one} on DIV2K \cite{Agustsson_2017_CVPR_Workshops} by approximately 2 dB and on RealSR \cite{realsr_cai2019toward} and DRealSR \cite{drealsr_wei2020component} by about 3 dB. These results underscore the efficiency and adaptability of our LoRA-based approach, which achieves superior fidelity and perceptual quality with substantially fewer parameters than these heavier diffusion models.

\begin{figure*}[t!]
\centering
\begin{subfigure}{0.26\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020hr_with_rectangle.pdf} \vspace{-8pt}\\ \centering \scriptsize DIV2K \cite{Agustsson_2017_CVPR_Workshops} - 804 (patch 00020) \\ ( / )
    \end{subfigure}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031hr_with_rectangle.pdf} \vspace{-8pt}\\ \centering \scriptsize RealSR \cite{realsr_cai2019toward} - Nikon 27  \\ ( /)
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020hr_crop.pdf} \vspace{-8pt}\\ \centering \scriptsize HR Crop \\ ( / )
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020osediff.pdf} \vspace{-8pt}\\ \centering \scriptsize OSEDiff \cite{lora_diff_realsr_wu2024one} \\ ( / )
    \end{subfigure}
     \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031hr_crop.pdf} \vspace{-8pt}\\ \centering \scriptsize HR Crop  \\ ( / )
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031osediff.pdf} \vspace{-8pt}\\ \centering \scriptsize OSEDiff \cite{lora_diff_realsr_wu2024one} \\ ( / )
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020ldl_swinir.pdf}
        \vspace{-8pt}\\ \centering \scriptsize LDL \cite{liang2022details} \\ ( / )
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020safmn_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SAFMN+LoRA \\ ( / )
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031ldl_swinir.pdf}
        \vspace{-8pt}\\ \centering \scriptsize LDL \cite{liang2022details} \\ ( /)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031safmn_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SAFMN+LoRA \\ ( / )
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020safmn.pdf} \vspace{-8pt}\\\centering \scriptsize  Real SAFMN-L \cite{safmn_sun2023spatially} \\ ( /)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020swinir_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SwinIR + LoRA \\ (/ )
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031safmn.pdf} \vspace{-8pt}\\\centering \scriptsize  Real SAFMN-L \cite{safmn_sun2023spatially} \\ ( / )
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031swinir_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize SwinIR + LoRA \\ ( /)
    \end{subfigure}
\end{subfigure}
\begin{subfigure}{0.14\textwidth}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020pasd.pdf} \vspace{-8pt}\\\centering \scriptsize PASD \cite{} \\ ( /)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/0807_pch_00020drct_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize DRCT + LoRA \\ ( /)
    \end{subfigure}
        \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031pasd.pdf} \vspace{-8pt}\\\centering \scriptsize PASD \cite{} \\ ( /)
    \end{subfigure}
    \begin{subfigure}{\textwidth}
        \includegraphics[width=\textwidth]{visuals/Nikon_031drct_lora.pdf} \vspace{-8pt}\\ \centering \scriptsize DRCT + LoRA \\ ( /)
    \end{subfigure}
\end{subfigure}
\vspace{-3pt}
\caption{Visual comparison of the proposed LoRA-enhanced models with the state-of-the-art methods for $\times$4 real SR. GAN and diffusion models fail to capture the content of images, exhibit excessive sharpness with color shifts. On the other hand, our LoRA-based models reconstruct high-fidelity details with correct alignment, particularly in complex areas with regular patterns. Additional visual comparisons can be found in the supplementary materials.}
\label{fig:qual_results} 
\end{figure*}

\noindent
\textbf{Qualitative Performance}
\label{sec:qual}
Figure \ref{fig:qual_results} illustrates visual comparisons among $\times$4 real SR methods, emphasizing the strengths of our LoRA-based domain-adapted approach. The qualitative results align closely with quantitative outcomes, revealing that GAN-SR models like LDL \cite{liang2022details} and SAFMN-Large \cite{safmn_sun2023spatially} often introduce artifacts, such as misaligning the roof’s striped patterns or even failing to capture accurate orientations. Similarly, diffusion-based methods like PASD \cite{yang2023pasd} and OSEDiff \cite{lora_diff_realsr_wu2024one} show excessive sharpness with content inaccuracies, incorrectly rendering structure and colors, for both images. In contrast, our LoRA-based models successfully reconstruct fine details, accurately aligning roof stripes and preserving the correct structure and colors in the second image to match the HR reference. Overall, our approach effectively controls artifacts while maintaining image fidelity, producing photorealistic, high-quality results in domain adaptation from bicubic to real SR.


% Figure \ref{fig:qual_results} illustrates visual comparisons among $\times$4 real SR approaches, highlighting the strengths of our LoRA-based domain adapted methods. Qualitative assessments closely align with the quantitative results, showing that GAN-SR models, including LDL \cite{liang2022details} and SAFMN-Large \cite{safmn_sun2023spatially}, often introduce artifacts, such as blending the man’s nose with the background or failing to reproduce textures. Similarly, diffusion-based methods like PASD \cite{yang2023pasd} and OSEDiff \cite{lora_diff_realsr_wu2024one} exhibit excessive sharpness with content inaccuracies, omitting details like the man’s mustache or failing to recover textures in the second patch. In contrast, our LoRA-based models adeptly reconstruct high-fidelity details, particularly in complex areas with regular patterns, such as retaining the man’s mustache and restoring textures in the second patch to match the HR image. Overall, our approach demonstrates a strong capacity to control artifacts while preserving accurate image details, achieving photorealistic, high-quality results in domain adaptation from bicubic to real SR.

\subsection{Ablation Study}
\label{sec:rank}
\noindent
\textbf{Rank Analysis.}
To identify the optimal LoRA rank for real SR adaptation, we conduct an ablation study by incrementally testing ranks from \( r = 1 \) to 64. Performance on the RealSR dataset for $\times$4 images, shown in Table \ref{table:rank_analysis}, demonstrates that even at rank 1 (with only 1.4$\%$ of the trainable parameters), the results closely match those from fine-tuning with 12M parameters. Optimal fidelity for PSNR and SSIM and perceptual quality for LPIPS are achieved at \( r = 8 \). Higher ranks (16 and 64) do not yield additional gains but still outperform full fine-tuning with fewer parameter updates. These results align with prior findings of \cite{zeng2023expressive}, suggesting that larger models often require lower LoRA ranks for effective adaptation, especially when pre-trained models are well-suited to the target task. This highlights LoRA’s efficiency in achieving efficient adaptation for even 1.4$\%$ parameter updates.

\begin{table}
 \caption{\textbf{Rank analysis} for better domain adaptation on RealSR \cite{realsr_cai2019toward} for 10k iterations. The best and the second-best are marked in \textbf{bold} and \underline{underlined}, respectively.} 
    \centering
    \scalebox{0.75}{
    \begin{tabular}{ccccccl}
    \specialrule{.1em}{.05em}{.05em} 
    Model & PSNR & SSIM & LPIPS & DISTS & Updated Paramaters\\  
    \hline
    Baseline & 27.5537& 0.7738& 0.3965& 0.2426 & 12M \\
    Baseline +FT & 28.2637& 0.7922& 0.3016& 0.2274 & +12M \\
    \hdashline
    r=1 &28.3383& 0.7957& 0.2772& 0.2129 &+152k (1.4\%)\\ 
    r=4 & 28.2675& 0.7945& 0.2721& \textbf{0.2125} & +466k (4.2\%)\\ 
    r=8 & \textbf{28.3999}& \textbf{0.7976}&\textbf{ 0.2705}& \textit{0.2128} & +886k (8.1\%)\\ 
    r=16 &\textit{28.3575}& \textit{0.7959}& 0.2719& 0.2140& +1.7M (15.5\%)\\ 
    r=64 & 28.3537& \textit{0.7959}& \textit{0.2716}& 0.2130 & +6.8M (61.8\%)\\ 
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:rank_analysis}
\end{table}

\noindent
\textbf{Extention to GAN-Based Real SR}
We further extend LoRA-based domain adaptation to GAN-based SR, showcasing its flexibility and efficiency. Using SwinIR \cite{liang2021swinir} with LoRA layers and a U-Net discriminator with spectral normalization \cite{wang2021real}, we apply adversarial training with a weighted combination of L1, perceptual \cite{johnson2016perceptual}, and GAN losses (1:1:0.1) as in RealESRGAN. As shown in Table \ref{table:gan_result}, our approach surpasses RealESRGAN \cite{wang2021real} and LDL \cite{liang2022details} in both fidelity and perceptual quality while using just 886k parameters, compared to 12M and 17M in LDL and RealESRGAN, respectively. These results highlight LoRA's capacity to tackle real-world degradations efficiently with minimal computational overhead. 

\begin{table}
 \caption{\textbf{Comparison of GAN-based RealSR }methods and our LoRA-enhanced SwinIR GAN method on DIV2K \cite{Agustsson_2017_CVPR_Workshops} validation patches. Our method achieves superior fidelity and perceptual quality with significantly fewer parameters.}
    \centering
    \scalebox{0.75}{
    \begin{tabular}{cccccc}
    \specialrule{.1em}{.05em}{.05em} 
    \multirow{2}{*}{GAN Method} & \multirow{2}{*}{PSNR $\uparrow$ } & \multirow{2}{*}{SSIM $\uparrow$} & \multirow{2}{*}{LPIPS $\downarrow$} & \multirow{2}{*}{DISTS $\downarrow$} & Trainable \\
    & & & & & Parameters\\ 
    \hline
   LDL (RealSwinIR) & 23.7565& 0.6403& 0.3091& 0.2189 & 12M \\
   RealESRGAN  & 21.94 & 0.5736 & 0.3868 & 0.260 & 17M \\
   SwinIR+LoRA  & 24.1093& 0.6598& 0.2914& 0.2085 & 886k \\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:gan_result}
\end{table}

==> sec/introo.tex <==
Image super-resolution (SR) is a critical task in computer vision, aimed at reconstructing high-resolution (HR) images from their low-resolution (LR) counterparts. It has diverse applications, spanning medical imaging \cite{medical_sr_isaac2015super, medical_sr_qiu2023medical} and satellite imaging \cite{satelite_sr_chen2023large, satelite_sr_karwowska2022using}, where image clarity is crucial. Traditional SR approaches \cite{dong2015image, kim2016accurate, johnson2016perceptual, ledig2017photorealistic, EDSR2017, srcnn, RCAN2018, wang2018esrgan, zhang2021ranksrgan} rely on simplified degradation models, such as bicubic downsampling, and prioritize architectural innovations. However, these models often fail to generalize to unknown or complex degradations due to their reliance on simplified assumptions.

While bicubic-trained SR models excel in handling bicubic degradations \cite{EDSR2017, RCAN2018, wang2018esrgan, zhang2018residual, niu_han, liang2021swinir, cat_chen2022cross, attention_zhang2022efficient, transformer_Chen_2023_ICCV, chen2023activating, korkmaz2024wavelettention}, their performance significantly deteriorates when applied to real-world images. Fine-tuning pre-trained models on real-world data can improve results \cite{wang2018esrgan, liang2022details}, but it is computationally prohibitive, requiring substantial memory and training time, which limits scalability and deployability, particularly on resource-constrained devices.

Some methods focus on explicitly training SR models for real-world data. GAN-based approaches \cite{ian_gan, wang2018esrgan, wang2021real}, specifically designed for real-world scenarios, leverage texture, color, and structural priors from pre-trained models \cite{lpips}, achieving promising results but often suffering from artifacts and instability in diverse scenes. Similarly, diffusion models (DMs) \cite{kawar2022denoising, ho2020denoising, dhariwal2021diffusion, ldm_rombach2022high, yang2023pixel, wang2024exploiting} have been explicitly trained on large-scale datasets, embedding natural image priors and demonstrating state-of-the-art performance. However, their multi-step processes introduce high computational costs, while recent one-step diffusion models \cite{lora_diff_realsr_wu2024one, lora_diff_realsr_wu2024seesr} improve efficiency, but sacrifice detail quality. These challenges highlight two critical research questions: 1. \textit{Can bicubically trained models generalize to real-world scenarios without expensive fine-tuning on real-world data?}, and 2. \textit{Can a computationally efficient model outperform existing GAN and diffusion-based approaches for real-world SR?}

To address the aforementioned issues, we propose a memory-efficient domain adaptation approach that leverages low-rank adaptation (LoRA) \cite{lora_orig_hu2021lora} to enable powerful domain shifts from bicubic to real-world image degradations in SR models. Unlike traditional fine-tuning methods, which require updating 100$\%$ of model weights and typically take days of training, our approach uses LoRA layers to minimize memory usage and computational demands. By updating only 8$\%$ of the model parameters, LoRA significantly reduces training time to just

==> sec/unused_data.tex <==
\begin{table*}
 \caption{Quantitative comparison of the proposed Low-Rank adaptation from bicubic domain to real SR methods representing the generalization capability of domain adaptation of LoRA SR. The best and the second-best results of each metric are highlighted in red and blue, respectively.
 }
    \centering
    \scalebox{0.85}{
    \begin{tabular}{llcccccccc}
    \specialrule{.1em}{.05em}{.05em} 
     Datasets &  Methods & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & DISTS $\downarrow$ &  CLIPIQA$\uparrow$& NIQE$\downarrow$ & MUSIQ$\uparrow$ &  MANIQA$\uparrow$\\
    \hline
     & RealESRGAN & 21.94 & 0.5736 & 0.3868 & 0.2601 & 4.9209 & 0.5251 & 58.64 & 0.5424 \\
     & LDL (RealESRGAN) & 23.8277& 0.6344& 0.3256& 0.2227& 0.5179& 4.8551& 60.0393& 0.5328 \\
     & LDL (RealSwinIR) & 23.7565& 0.6403& 0.3091& 0.2189& 0.4884& 4.9317& 57.2523& 0.5260 \\
      & Real-SAFMN-L & 23.2124& 0.5950& 0.3282& 0.2153& 0.6552& 4.1064& 64.9999& 0.5691 \\
    \hdashline
     & StableSR & 23.26 & 0.5726 & 0.3113 & 0.2048 & 0.6771 & 4.7581 & 65.92 & 0.6192 \\
     & SeeSR & 23.68 & 0.6043 & 0.3194 & 0.1968 & 0.6936 & 4.8102 & 68.67 & 0.6240 \\
     & PASD & 23.14 & 0.5505 & 0.3571 & 0.2207 & 0.6788 & 4.3617 & 68.95 & 0.6483\\
     & SinSR & 24.41 & 0.6018 & 0.3240 & 0.2066 & 0.6471 & 6.0159 & 62.82 & 0.5386 \\
\textit{ DIV2K} & OSEDiff & 23.72 & 0.6108 & 0.2941 & 0.1976 & 0.6683 & 4.7097 & 67.97 & 0.6148 \\
 \hdashline
     & EDSR & 24.9164& 0.6261& 0.6740& 0.3304& 0.3050& 9.3819& 22.6555& 0.3225 \\
     & EDSR+LoRA& 25.5393& 0.6553& 0.5376& 0.3324& 0.2399& 9.2358& 33.9969& 0.2460\\
     & SAFMN & 24.9298& 0.6264& 0.6758& 0.3308& 0.3220& 9.4724& 22.3746& 0.3252\\
     & SAFMN+LoRA & 25.4742& 0.6547& 0.5461& 0.3271& 0.2113& 8.9846& 32.0203& 0.2476\\
     & SwinIR & 24.8738& 0.6237& 0.6731& 0.3305& 0.3044& 9.2404& 22.6681& 0.3213 \\
     &  SwinIR+LoRA &25.8058& 0.6681& 0.5047& 0.3194& 0.2792& 9.1162& 39.0488& 0.2686 \\
     & DRCT & 24.8938& 0.6249& 0.6744& 0.3301& 0.3124& 9.3966& 22.8727& 0.3240\\
     &  DRCT+LoRA &25.7739& 0.6693& 0.5037& 0.3167& 0.2768& 9.0199& 38.6876& 0.2647 \\
     \hline
     & RealESRGAN & 25.69 & 0.7616 & 0.2727 & 0.2063 & 0.4449 & 5.8295 & 60.82 & 0.5485\\
     & LDL (RealESRGAN) &25.2805& 0.7565& 0.2750& 0.2120& 0.4557& 5.9933& 60.9320& 0.5495 \\
     & LDL (RealSwinIR) & 24.9640& 0.7634& 0.2519& 0.1981& 0.4297& 6.1917& 58.0443& 0.5279\\
     & Real-SAFMN-L & 24.2288& 0.7217& 0.2905& 0.2176& 0.5857& 4.8866& 66.3470& 0.5894 \\
    \hdashline
     & StableSR & 24.70 & 0.7085 & 0.3018 & 0.2288 & 0.6178 & 5.9122 & 65.78 & 0.6221 \\
     & SeeSR & 25.18& 0.7216& 0.3009& 0.2223& 0.6612& 5.4081& 69.77& 0.6442\\
     & PASD & 25.21& 0.6798& 0.3380& 0.2260& 0.6620& 5.4137& 68.75& 0.6487\\
     & SinSR & 26.28& 0.7347& 0.3188& 0.2353& 0.6122& 6.2872& 60.80& 0.5385\\
 \textit{RealSR} & OSEDiff &25.15& 0.7341& 0.2921& 0.2128& 0.6693& 5.6476& 69.09& 0.6326\\
 \hdashline
     & EDSR & 27.5422& 0.7732& 0.3937& 0.2436& 0.3289& 8.3179& 30.8765& 0.3642 \\
     & EDSR+LoRA & 27.9260& 0.7878& 0.2835& 0.2190& 0.2829& 7.8546& 43.9013& 0.3766\\
     & SAFMN &27.5583& 0.7740& 0.3927& 0.2430& 0.3338& 8.3443& 30.7043& 0.3703\\
     & SAFMN+LoRA & 28.3245& 0.7935& 0.2935& 0.2229& 0.2614& 7.7209& 41.8672& 0.3780 \\
     & SwinIR &27.5537& 0.7738& 0.3965& 0.2426& 0.3388& 8.3294& 30.5589& 0.3711 \\
     &  SwinIR+LoRA & 28.6964& 0.8079& 0.2591& 0.2109& 0.3264& 8.3661& 48.4967& 0.3947 \\
     & DRCT & 27.5502& 0.7737& 0.3966& 0.2434& 0.3384& 8.3130& 30.5884& 0.3671 \\
     &  DRCT+LoRA & 28.7173& 0.8061& 0.2553& 0.2094& 0.3206& 8.3144& 48.0846& 0.3968 \\
\hline
     & RealESRGAN & 28.64 & 0.8053 & 0.2847 & 0.2089 & 0.4422 & 6.6928 & 54.18 &  0.4907\\
     & LDL (RealESRGAN) &28.1960& 0.8124& 0.2792& 0.2127& 0.4476& 7.1430& 53.9484& 0.4894\\
     & LDL (RealSwinIR) &27.4297& 0.8078& 0.2655& 0.2055& 0.4411& 6.9388& 52.3765& 0.4833\\
     & Real-SAFMN-L & 27.1494& 0.7671& 0.3148& 0.2219& 0.6319& 5.4987& 61.8574& 0.5518\\
 \hdashline
     & StableSR & 28.03 & 0.7536 & 0.3284 & 0.2269 & 0.6356 & 6.5239 & 58.51 & 0.5601\\
     & SeeSR & 28.17& 0.7691& 0.3189& 0.2315& 0.6804& 6.3967& 64.93& 0.6042\\
     & PASD &27.36& 0.7073& 0.3760& 0.2531& 0.6808 & 5.5474& 64.87& 0.6169\\
     & SinSR & 28.36& 0.7515& 0.3665& 0.2485 & 0.6383& 6.9907& 55.33& 0.4884 \\
    \textit{DRealSR} & OSEDiff &27.9243& 0.7835& 0.2968& 0.2165& 0.6963& 6.4902& 64.6537& 0.5899\\
    \hdashline
     & EDSR &30.6469& 0.8328& 0.4364& 0.2695& 0.3453& 10.3217& 24.0425& 0.3202\\
     & EDSR+LoRA &30.6370& 0.8368& 0.3523& 0.2548& 0.2678& 9.5520& 34.1941& 0.2861 \\
     & SAFMN &30.6221& 0.8327& 0.4356& 0.2689& 0.3486& 10.2994& 24.0977& 0.3212 \\
     & SAFMN+LoRA & 30.9162& 0.8403& 0.3529& 0.2545& 0.2384& 9.3912& 33.4356& 0.2976\\
     & SwinIR & 30.6209& 0.8327& 0.4391& 0.2708& 0.3556& 10.4489& 24.2130& 0.3254\\
     & SwinIR+FT & 30.8027& 0.8400& 0.3565& 0.2565& 0.2843& 9.3757& 32.4649& 0.2958\\
     &  SwinIR+LoRA & 30.7392& 0.8422& 0.3381& 0.2524& 0.3127& 10.0046& 37.4812& 0.2839\\
     & DRCT & 30.6066& 0.8325& 0.4394& 0.2703& 0.3533& 10.3466& 24.1620& 0.3236 \\
     &  DRCT+LoRA &30.8109& 0.8419& 0.3414& 0.2544& 0.3107& 10.0394& 36.9073& 0.2885\\

\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_arc_lora}
\end{table*}

\begin{table*}
 \caption{Quantitative comparison of the proposed Low-Rank adaptation from bicubic domain to real SR methods representing the generalization capability of domain adaptation of LoRA SR. The best and the second-best results of each metric are highlighted in red and blue, respectively.
 }
    \centering
    \scalebox{0.85}{
    \begin{tabular}{l|llccccc}
    \specialrule{.1em}{.05em}{.05em} 
     Datasets &  & Methods & Trainable Parameters & PSNR $\uparrow$ & SSIM $\uparrow$ & LPIPS $\downarrow$ & DISTS $\downarrow$ \\
    \hline
    % & \multirow{4}{*}{\rotatebox[origin=c]{90}{\parbox{2mm} {\centering GAN-Based}}} & RealESRGAN & 17M & 21.94 & 0.5736 & 0.3868 & 0.260\\
    \multirow{13}{*}{\centering\textit{ DIV2K}} & \multirow{4}{*}{\centering GAN-Based} & RealESRGAN & 17M & 22.94 & 0.6036 & 0.3768 & 0.2520\\
    % & & RealESRGAN & 17M & 21.94 & 0.5736 & 0.3868 & 0.2601 \\
    & & LDL (RealESRGAN) & 17M & 23.8277& 0.6344& 0.3256& 0.2227 \\
    & & LDL (RealSwinIR)& 12M & 23.7565& 0.6403& 0.3091& 0.2189 \\
    &  & Real-SAFMN-L & 5.6M & 23.2124& 0.5950& 0.3282& 0.2153 \\
    \hdashline
    & \multirow{5}{*}{\centering Diffusion-Based} &  StableSR & 150M & 23.26 & 0.5726 & 0.3113 & 0.2048  \\
    & & SeeSR & 750M & 23.68 & 0.6043 & 0.3194 & 0.1968 \\
    & & PASD & 625M & 23.14 & 0.5505 & 0.3571 & 0.2207 \\
    & & SinSR & 119M & 24.41 & 0.6018 & 0.3240 & 0.2066 \\
    & & OSEDiff & 8.5M & 23.72 & 0.6108 & 0.2941 & 0.1976 \\
 \hdashline
    & \multirow{4}{*}{\centering Ours} & EDSR+LoRA& 314k & 25.5393& 0.6553& 0.5376& 0.3324 \\
    & & SAFMN+LoRA & 99.5k & 25.4742& 0.6547& 0.5461& 0.3271 \\
    & &  SwinIR+LoRA & 886k & 25.8058& 0.6681& 0.5047& 0.3194 \\
    & &  DRCT+LoRA & 3.1M & 25.7739& 0.6693& 0.5037& 0.3167  \\
     \hline
   \multirow{13}{*}{\centering\textit{RealSR}} & \multirow{4}{*}{\centering GAN-Based} & RealESRGAN & 17M & 25.69 & 0.7616 & 0.2727 & 0.2063 \\
    & & LDL (RealESRGAN) & 17M &25.2805& 0.7565& 0.2750& 0.2120 \\
    & & LDL (RealSwinIR) & 12M & 24.9640& 0.7634& 0.2519& 0.1981 \\
    & & Real-SAFMN-L & 5.6M & 24.2288& 0.7217& 0.2905& 0.2176 \\
    \hdashline
    & \multirow{5}{*}{\centering Diffusion-Based} & StableSR & 150M & 24.70 & 0.7085 & 0.3018 & 0.2288 \\
    & & SeeSR & 750M & 25.18& 0.7216& 0.3009& 0.2223\\
    & & PASD & 625M &25.21& 0.6798& 0.3380& 0.2260 \\
    & & SinSR & 119M & 26.28& 0.7347& 0.3188& 0.2353\\
    & & OSEDiff & 8.5M &25.15& 0.7341& 0.2921& 0.2128 \\
 \hdashline
    & \multirow{4}{*}{\centering Ours} & EDSR+LoRA &314k & 27.9260& 0.7878& 0.2835& 0.2190 \\
     & & SAFMN+LoRA & 99.5k & 28.3245& 0.7935& 0.2935& 0.2229 \\
     & &  SwinIR+LoRA & 886k & 28.6964& 0.8079& 0.2591& 0.2109 \\
     & &  DRCT+LoRA & 3.1M &  28.7173& 0.8061& 0.2553& 0.2094 \\
\hline
     \multirow{13}{*}{\centering\textit{ DRealSR}} & \multirow{4}{*}{\centering GAN-Based} & RealESRGAN & 17M & 28.64 & 0.8053 & 0.2847 & 0.2089\\
     & & LDL (RealESRGAN) & 17M &28.1960& 0.8124& 0.2792& 0.2127 \\
     & & LDL (RealSwinIR) & 12M & 27.4297& 0.8078& 0.2655& 0.2055 \\
     & & Real-SAFMN-L & 5.6M & 27.1494& 0.7671& 0.3148& 0.2219 \\
 \hdashline
     & \multirow{5}{*}{\centering Diffusion-Based} & StableSR & 150M & 28.03 & 0.7536 & 0.3284 & 0.2269 \\
     & & SeeSR & 750M & 28.17& 0.7691& 0.3189& 0.2315 \\
     & & PASD & 625M &27.36& 0.7073& 0.3760& 0.2531 \\
     & & SinSR & 119M & 28.36& 0.7515& 0.3665& 0.2485 \\
     & & OSEDiff & 8.5M &27.9243& 0.7835& 0.2968& 0.2165 \\
    \hdashline
     & \multirow{4}{*}{\centering Ours} & EDSR+LoRA & 314k & 30.6370& 0.8368& 0.3523& 0.2548 \\
     & & SAFMN+LoRA & 99.5k & 30.9162& 0.8403& 0.3529& 0.2545 \\
     & &  SwinIR+LoRA & 886k & 30.7392& 0.8422& 0.3381& 0.2524 \\
     & & DRCT+LoRA & 3.1M &30.8109& 0.8419& 0.3414& 0.2544 \\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:diff_arc_lora_2}
\end{table*}


\begin{table*}
 \caption{DIV2K + DrealSR}
    \centering
    \scalebox{0.9}{
    \begin{tabular}{ccccccccc}
    \specialrule{.1em}{.05em}{.05em} 
     Metric & EDSR & EDSR+LoRA & SAFMN & SAFMN+LoRA & SwinIR & SwinIR+LoRA & DRCT & DRCT+LoRA \\ 
     \hline
    PSNR $\uparrow$ & 24.9164& 25.5393& 24.9298& 25.4742& 24.8738& 25.8058& 24.8938& 25.7739 \\
    SSIM $\uparrow$ &  0.6261& 0.6553& 0.6264& 0.6547& 0.6237& 0.6681& 0.6249& 0.6693 \\ 
    LPIPS $\downarrow$ &  0.6740& 0.5376& 0.6758& 0.5461& 0.6731& 0.5047& 0.6744& 0.5037 \\
    DISTS $\downarrow$ &  0.3304& 0.3324& 0.3308& 0.3271& 0.3305& 0.3194& 0.3301& 0.3167 \\ 
    CLIPIQA$\uparrow$&  0.3050& 0.2399& 0.3220& 0.2113& 0.3044& 0.2792& 0.3124& 0.2768 \\
    NIQE$\downarrow$ &  9.3819& 9.2358& 9.4724& 8.9846& 9.2404& 9.1162& 9.3966& 9.0199 \\
    MUSIQ$\uparrow$ &  22.6555& 33.9969& 22.3746& 32.0203& 22.6681& 39.0488& 22.8727& 38.6876 \\
    MANIQA $\uparrow$ &  0.3225 & 0.2460 & 0.3252 & 0.2476 & 0.3213 & 0.2686 & 0.3240 & 0.2647 \\
    \hline
    PSNR $\uparrow$ & 30.6469& 30.6370& 30.6221& 30.9162& 30.6209& 30.7392& 30.6066& 30.8109\\
    SSIM $\uparrow$ &  0.8328& 0.8368& 0.8327& 0.8403& 0.8327& 0.8422& 0.8325& 0.8419 \\
    LPIPS $\downarrow$ & 0.4364& 0.3523& 0.4356& 0.3529& 0.4391& 0.3381& 0.4394& 0.3414\\
    DISTS $\downarrow$ &  0.2695& 0.2548& 0.2689& 0.2545& 0.2708& 0.2524& 0.2703& 0.2544 \\ 
    CLIPIQA$\uparrow$& 0.3453& 0.2678& 0.3486& 0.2384& 0.3556& 0.3127& 0.3533& 0.3107\\
    NIQE$\downarrow$ & 10.3217& 9.5520& 10.2994& 9.3912& 10.4489& 10.0046& 10.3466& 10.0394 \\
    MUSIQ$\uparrow$ &  24.0425& 34.1941& 24.0977& 33.4356& 24.2130& 37.4812& 24.1620& 36.9073 \\
    MANIQA $\uparrow$ &  0.3202 & 0.2861 & 0.3212 & 0.2976 & 0.3254 & 0.2839 & 0.3236 & 0.2885\\
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:domain_adaptation}
\end{table*}

\begin{table}
 \caption{Rank analysis. 10k iter, realsr val The best and the second-best are marked in \textbf{bold} and \underline{underlined}, respectively.}
    \centering
    \scalebox{0.75}{
    \begin{tabular}{ccccccl}
    \specialrule{.1em}{.05em}{.05em} 
    Model & PSNR & SSIM & LPIPS & DISTS & Updated Paramaters\\  
    \hline
    Baseline & 27.5537& 0.7738& 0.3965& 0.2426 & 12M \\
    Baseline +FT & 28.2637& 0.7922& 0.3016& 0.2274 & +12M \\
    \hdashline
    r=1 &28.3383& 0.7957& 0.2772& 0.2129 &+152k (1.4\%)\\ 
    r=2 &28.3515& 0.7968& 0.2723& 0.2123 & +257k (2.4\%)\\ 
    r=4 & 28.2675& 0.7945& 0.2721& 0.2125 & +466k (4.2\%)\\ 
    r=8 & 28.3999& 0.7976& 0.2705& 0.2128 & +886k (8.1\%)\\ 
    r=16 &28.3575& 0.7959& 0.2719& 0.2140& +1.7M (15.5\%)\\ 
    r=32 &28.2317& 0.7930& 0.2723& 0.2132&  +3.4M (30.9\%)\\ (25.272/0.964)

    r=64 & 28.3537& 0.7959& 0.2716& 0.2130 & +6.8M (61.8\%)\\ 
\specialrule{.1em}{.05em}{.05em} 
    \end{tabular} 
}
\label{table:rank_analysis}
\end{table}

\begin{figure}
\centering
\includegraphics[width=\linewidth]{images/cos_sim_weights.png}
\caption{?}
\label{fig:cos_sim_weights}
\end{figure}

while LoRA itself is indeed a known technique, our work goes beyond simply applying it to SR. Specifically, we’ve conducted a deep analysis to determine where and how LoRA should be integrated into SR models for effective domain adaptation—examining which modules (like convolutional, attention, and MLP layers) yield the best trade-offs in performance, memory efficiency, and computational overhead.

Furthermore, we’ve developed strategies for LoRA integration that make SR models adaptable from bicubic to real-world degradations, achieving comparable or better results than full fine-tuning with significantly fewer parameters. This approach isn’t just a plug-and-play application; it's about understanding LoRA’s potential within SR, optimizing it for complex degradations, and rigorously validating its advantages across different SR architectures. The novelty lies in the tailored application, the efficiency gains, and the comprehensive evaluation of LoRA for SR-specific tasks and real-world scenarios.
